Using Large Language Models for Interpreting Autonomous Robots Behaviors

The deployment of autonomous robots in various domains has raised significant concerns about their trustworthiness and accountability. This study explores the potential of Large Language Models (LLMs) in analyzing ROS 2 logs generated by autonomous robots and proposes a framework for log analysis that categorizes log files into different aspects. The study evaluates the performance of three different language models in answering questions related to StartUp, Warning, and PDDL logs. The results suggest that GPT 4, a transformer-based model, outperforms other models, however, their verbosity is not enough to answer why or how questions for all kinds of actors involved in the interaction.

==> assets/casoPDDL_antesLimpieza.tex <==

\begin{tiny}
\begin{tcolorbox}
\begin{multicols}{2}
\begin{verbatim}
** Domain **
.7237854 [exec-node-8] [INFO] [.723554341] 
        [merlin2.executor_node]: 
        (define (domain merlin2)
.7239003 [exec-node-8] 
        (:requirements :typing 
        :negative-preconditions :durative-actions)
.7239411 [exec-node-8] (:types
.7239749 [exec-node-8] 	door
.7240303 [exec-node-8] 	sound
.7240658 [exec-node-8] 	wp
.7240963 [exec-node-8] )
.7241285 [exec-node-8] (:predicates
.7241755 [exec-node-8] 	(door_at ?d0 - door ?w1 - wp)
.7242112 [exec-node-8] 	(door_checked ?d0 - door)
.7242436 [exec-node-8] 	(robot_at ?w0 - wp)
.7242765 [exec-node-8] 	(sound_listened ?s0 - sound)
.7243075 [exec-node-8] )
.7243369 [exec-node-8] (:durative-action check_door
.7243667 [exec-node-8] 	:parameters ( ?wp - wp ?door - door)
.7243962 [exec-node-8] 	:duration (= ?duration 10)
.7244265 [exec-node-8] 	:condition (and
.7244639 [exec-node-8] 		(at start (door_at ?door ?wp))
.7245104 [exec-node-8] 		(at start (robot_at ?wp))
.7245495 [exec-node-8] 	)
.7245889 [exec-node-8] 	:effect (and
.7246275 [exec-node-8] 		(at end (door_checked ?door))
.7246664 [exec-node-8] 	)
.7247052 [exec-node-8] )
.7247431 [exec-node-8] (:durative-action navigation
.7247810 [exec-node-8] 	:parameters ( ?o - wp ?d - wp)
.7248192 [exec-node-8] 	:duration (= ?duration 10)
.7248578 [exec-node-8] 	:condition (and
.7248914 [exec-node-8] 		(at start (robot_at ?o))
.7249236 [exec-node-8] 	)
.7249556 [exec-node-8] 	:effect (and
.7249880 [exec-node-8] 		(at end (robot_at ?d))
.7250199 [exec-node-8] 		(at start (not (robot_at ?o)))
.7250516 [exec-node-8] 	)  )  )
** Problem **
.7254245 [exec-node-8] 
            [INFO] [.723845161] [merlin2.executor_node]: 
            (define (problem merlin2_prb)
.7254870 [exec-node-8] (:domain merlin2)
.7255244 [exec-node-8] (:objects
.7255585 [exec-node-8] 	boiling - sound
.7255921 [exec-node-8] 	door_entrance - door
.7256258 [exec-node-8] 	doorbell - sound
.7256558 [exec-node-8] 	entrance - wp
.7256918 [exec-node-8] 	insect - sound
.7257254 [exec-node-8] 	inside_small_room - sound
.7257576 [exec-node-8] 	livingroom - wp
.7257905 [exec-node-8] 	mechanical_fan - sound
.7258232 [exec-node-8] 	music - sound
.7258549 [exec-node-8] 	rustle - sound
.7258875 [exec-node-8] 	tubular_bells - sound
.7259202 [exec-node-8] 	white_noise - sound
.7259526 [exec-node-8] )
.7259843 [exec-node-8] (:init
.7260165 [exec-node-8] 	(robot_at livingroom)
.7260485 [exec-node-8] 	(door_at door_entrance entrance)
.7260811 [exec-node-8] 	(sound_listened tubular_bells)
.7261131 [exec-node-8] )
.7261448 [exec-node-8] (:goal
.7261763 [exec-node-8] 	(and
.7262082 [exec-node-8] 	(door_checked door_entrance)
.7262411 [exec-node-8] 	(robot_at livingroom)
.7262723 [exec-node-8] 	)
.7263045 [exec-node-8] )
.7263389 [exec-node-8] )







\end{verbatim}
\end{multicols}
\end{tcolorbox}
\end{tiny}


The answers provided provided by the large language model (LLM) selected, with single shot is:
% \textcolor{orange}{

% ** GPT3.5 **
% Sure, here is a plan that satisfies the goal:

% makefile

% 0: check\_door livingroom door\_entrance
% 1: navigation livingroom entrance

% This plan checks the door at the entrance, and then 
% navigates to the entrance. By the end of the plan, the robot 
% is at the livingroom and the door at the entrance is checked.

% }

\begin{tiny}
\begin{multicols}{2}
\begin{alltt}


\textcolor{orange}{

** GPT3.5 **
Domain
It looks like the code you provided is written in the domain 
specification language of the PDDL (Planning Domain Definition 
Language), which is used for describing a planning domain in 
AI planning.

The code defines a domain named "merlin2" that requires the 
use of typing, negative preconditions, and durative actions. 
It then defines three types of objects: doors, sounds, and 
waypoints.

The domain also defines five predicates (door_at, door_checked, 
robot_at, sound_listened), which are used to represent the 
state of the planning domain.

Finally, the domain defines two durative actions: "check_door"
and "navigation". The "check_door" action has two parameters, 
a waypoint object, and a door object. It takes 10 units of 
time to execute and can only be executed if the robot is at 
the specified waypoint and the specified door is also at that 
same waypoint. The effect of the "check_door" action is to set
the checked state of the door to true.

The "navigation" action has two parameters, two waypoint 
objects representing the start and end points of a navigation 
task. This action also takes 10 units of time to execute and 
can only be executed if the robot is at the starting waypoint. 
The effect of the "navigation" action is to move the robot to t
he destination waypoint while setting the robot's previous location to false.

Problem:
It appears to be a snippet of code written in the PDDL (Planning 
Domain Definition Language) syntax. PDDL is a language used to 
define the planning problem and domain for AI planning systems.

The code defines a problem called "merlin2_prb" in the domain 
"merlin2". It defines several objects, including sounds, doors, 
and waypoints. It initializes the robot's location in the living 
room, the door's location at the entrance, and the sound listened 
to as tubular bells. Finally, it sets a goal for the robot to 
check the door and be in the living room.
}

** GPT 4 **
This PDDL problem is defined within the previously explained 
merlin2 domain. It specifies the objects, the initial state, 
and the goal for a specific problem instance.

Objects:

    Sounds: boiling, doorbell, insect, inside_small_room, 
    mechanical_fan, music, rustle, tubular_bells, white_noise
    Doors: door_entrance
    Waypoints: entrance, livingroom

Initial state:

    The robot is at the livingroom waypoint.
    The door_entrance is at the entrance waypoint.
    The robot has listened to the tubular_bells sound.

Goal state:

    The door_entrance must be checked by the robot.
    The robot must be at the livingroom waypoint.

As an AI language model, I am unable to run a planner to 
solve this problem directly. However, I can suggest a 
simple plan that could achieve the goal state based on 
the given domain and problem instance:

    Perform the navigation action:
        Parameters: ?o - livingroom, ?d - entrance
        This action moves the robot from the livingroom 
        to the entrance waypoint.

    Perform the check_door action:
        Parameters: ?wp - entrance, ?door - door_entrance
        This action checks the door_entrance while the 
        robot is at the entrance waypoint.

    Perform the navigation action again:
        Parameters: ?o - entrance, ?d - livingroom
        This action moves the robot back from the entrance 
        to the livingroom waypoint.

After executing these three actions, the robot would have
checked the door_entrance and returned to the livingroom 
waypoint, satisfying the specified goal conditions.

\textcolor{blue}{** ALPACA **

The log entry indicates that the robot is at its starting
position, which in this case was inside a small room with 
white noise playing and tubular bells ringing from outside 
of it (the door). The goal state for the agent to reach 
involved closing both doors. After reaching the goal, the 
agent then exited through one of them while listening to 
the sound played by its own robotic arm.

### Observation:
The observation log shows that tubular bells are playing 
outside and white noise is being generated inside a small 
room with no other objects in it (the door). The robot's 
position was also recorded as being at one of two doors, 
which were both open when the agent started its task. 

### Action:
The action log shows that the robotic arm moved to close 
each respective door and then played a sound from itself 
while listening for any response (the goal). After 
reaching this state successfully, it exited through 
either one of them depending on which was closer at the 
time when the agent started its task. 

### Effect:
The effect log shows that tubular bells are still playing 
outside and white noise is being generated inside a small 
room with no other objects in it (the door). The robot
}
\end{alltt}

\end{multicols}
\end{tiny}

==> assets/launch_log.tex <==
1678884557.6391342 [INFO] [launch]: All log files can be found below /home/gentlebots/.ros/log/2023-03-15-13-49-17-632183-gentlebots-116634
1678884557.6392949 [INFO] [launch]: Default logging verbosity is set to INFO
1678884558.4071975 [INFO] [waypoint_navigation_node-1]: process started with pid [116636]
1678884558.4074376 [INFO] [sound_recognition_node-2]: process started with pid [116638]
1678884558.4075477 [INFO] [manager_node-3]: process started with pid [116640]
1678884558.4076343 [INFO] [tts_node-4]: process started with pid [116642]
1678884558.4077158 [INFO] [pddl_generator_node-5]: process started with pid [116644]
1678884558.4081540 [INFO] [planner_node-6]: process started with pid [116646]
1678884558.4095747 [INFO] [plan_dispatcher_node-7]: process started with pid [116648]
1678884558.4109290 [INFO] [executor_node-8]: process started with pid [116650]
1678884558.4122808 [INFO] [merlin2_listen_audio_node-9]: process started with pid [116652]
1678884558.4136653 [INFO] [merlin2_navigation_fsm_action-10]: process started with pid [116654]
1678884558.4150121 [INFO] [merlin2_check_door_fsm_action-11]: process started with pid [116656]
1678884558.4447975 [INFO] [merlin2_demo3_node-12]: process started with pid [116658]
1678884559.4909811 [tts_node-4] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6102691 [merlin2_check_door_fsm_action-11] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6540756 [planner_node-6] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.8783755 [manager_node-3] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.1545579 [waypoint_navigation_node-1] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3826396 [executor_node-8] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3833480 [pddl_generator_node-5] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.4762170 [waypoint_navigation_node-1] /opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py:441: UserWarning: when declaring parameter named 'wps', declaring a parameter only providing its name is deprecated. You have to either:
1678884560.4764743 [waypoint_navigation_node-1] 	- Pass a name and a default value different to "PARAMETER NOT SET" (and optionally a descriptor).
1678884560.4766202 [waypoint_navigation_node-1] 	- Pass a name and a parameter type.
1678884560.4767292 [waypoint_navigation_node-1] 	- Pass a name and a descriptor with `dynamic_typing=True
1678884560.4768608 [waypoint_navigation_node-1]   warnings.warn(
1678884560.4823425 [merlin2_demo3_node-12] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.5726750 [plan_dispatcher_node-7] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6693683 [merlin2_listen_audio_node-9] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6927030 [merlin2_navigation_fsm_action-10] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884561.2024031 [merlin2_demo3_node-12] [INFO] [1678884561.202155833] [merlin2.merlin2_demo3_node]: Waiting for doorbell...
1678884561.2941566 [sound_recognition_node-2] 2023-03-15 13:49:21.293771: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884561.2943850 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884561.5250556 [sound_recognition_node-2] 2023-03-15 13:49:21.524792: I tensorflow/core/util/port.cc:104] oneDNN custom operations are on. You may see slightly different numerical results due to floating-point round-off errors from different computation orders. To turn them off, set the environment variable `TF_ENABLE_ONEDNN_OPTS=0`.
1678884561.5278707 [sound_recognition_node-2] 2023-03-15 13:49:21.527592: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcudart.so.11.0'; dlerror: libcudart.so.11.0: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884561.5280049 [sound_recognition_node-2] 2023-03-15 13:49:21.527611: I tensorflow/compiler/xla/stream_executor/cuda/cudart_stub.cc:29] Ignore above cudart dlerror if you do not have a GPU set up on your machine.
1678884562.4255106 [sound_recognition_node-2] 2023-03-15 13:49:22.425286: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer.so.7'; dlerror: libnvinfer.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4259348 [sound_recognition_node-2] 2023-03-15 13:49:22.425422: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer_plugin.so.7'; dlerror: libnvinfer_plugin.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4260798 [sound_recognition_node-2] 2023-03-15 13:49:22.425431: W tensorflow/compiler/tf2tensorrt/utils/py_utils.cc:38] TF-TRT Warning: Cannot dlopen some TensorRT libraries. If you would like to use Nvidia GPU with TensorRT, please make sure the missing libraries mentioned above are installed properly.
1678884563.2107456 [sound_recognition_node-2] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884563.3666165 [sound_recognition_node-2] 2023-03-15 13:49:23.366304: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcuda.so.1'; dlerror: libcuda.so.1: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884563.3667796 [sound_recognition_node-2] 2023-03-15 13:49:23.366321: W tensorflow/compiler/xla/stream_executor/cuda/cuda_driver.cc:265] failed call to cuInit: UNKNOWN ERROR (303)
1678884563.3668425 [sound_recognition_node-2] 2023-03-15 13:49:23.366336: I tensorflow/compiler/xla/stream_executor/cuda/cuda_diagnostics.cc:156] kernel driver does not appear to be running on this host (gentlebots): /proc/driver/nvidia/version does not exist
1678884563.3672061 [sound_recognition_node-2] 2023-03-15 13:49:23.366532: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884563.3672807 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884564.7082698 [sound_recognition_node-2] [INFO] [1678884564.708041692] [sound_recognition.sound_recognition_node]: listen_thread starts listening
1678884564.7307980 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.front
1678884564.7310190 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.rear
1678884564.7310867 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.center_lfe
1678884564.7311323 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.side
1678884564.7312636 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313192 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313838 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround40
1678884564.7314229 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround41
1678884564.7318101 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround50
1678884564.7319388 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround51
1678884564.7319987 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround71
1678884564.7320669 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321129 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321570 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321966 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322392 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322824 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323217 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323618 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7326291 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7371376 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7373369 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7408085 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7409520 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7410004 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7410374 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7413969 [sound_recognition_node-2] ALSA lib pcm_dmix.c:1032:(snd_pcm_dmix_open) unable to open slave
1678884566.9160802 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 1s 841ms/step
1678884566.9175122 [sound_recognition_node-2] [INFO] [1678884566.917240165] [sound_recognition.sound_recognition_node]: music
1678884567.9730656 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884567.9741521 [sound_recognition_node-2] [INFO] [1678884567.973858829] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884568.0223629 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884568.0231643 [sound_recognition_node-2] [INFO] [1678884568.023020035] [sound_recognition.sound_recognition_node]: insect
1678884569.0709331 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884569.0717046 [sound_recognition_node-2] [INFO] [1678884569.071502259] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884570.3489144 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884570.3496821 [sound_recognition_node-2] [INFO] [1678884570.349498574] [sound_recognition.sound_recognition_node]: boiling
1678884571.6400306 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884571.6410005 [sound_recognition_node-2] [INFO] [1678884571.640862477] [sound_recognition.sound_recognition_node]: white_noise
1678884572.7147002 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884572.7157867 [sound_recognition_node-2] [INFO] [1678884572.715541398] [sound_recognition.sound_recognition_node]: rustle
1678884573.9964857 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884573.9973874 [sound_recognition_node-2] [INFO] [1678884573.997236108] [sound_recognition.sound_recognition_node]: inside_small_room
1678884574.0422242 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884574.0431235 [sound_recognition_node-2] [INFO] [1678884574.042970121] [sound_recognition.sound_recognition_node]: white_noise
1678884575.0656774 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884575.0665801 [sound_recognition_node-2] [INFO] [1678884575.066414965] [sound_recognition.sound_recognition_node]: white_noise
1678884576.3594229 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884576.3607428 [sound_recognition_node-2] [INFO] [1678884576.360408696] [sound_recognition.sound_recognition_node]: inside_small_room
1678884577.6447077 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884577.6457713 [sound_recognition_node-2] [INFO] [1678884577.645569064] [sound_recognition.sound_recognition_node]: tubular_bells
1678884577.6519880 [merlin2_demo3_node-12] [INFO] [1678884577.651800678] [merlin2.merlin2_demo3_node]: EXECUTING MISSION: Answer the door
1678884577.6523142 [merlin2_demo3_node-12] [INFO] [1678884577.652082970] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6556804 [merlin2_demo3_node-12] [INFO] [1678884577.655544354] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6559033 [merlin2_demo3_node-12] [INFO] [1678884577.655777629] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6604662 [merlin2_demo3_node-12] [INFO] [1678884577.660297157] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6607640 [merlin2_demo3_node-12] [INFO] [1678884577.660550771] [merlin2.merlin2_demo3_node]: goals saved
1678884577.6615767 [merlin2_demo3_node-12] [INFO] [1678884577.661483619] [merlin2.merlin2_demo3_node]: wait for results
1678884577.7237854 [executor_node-8] [INFO] [1678884577.723554341] [merlin2.executor_node]: (define (domain merlin2)
1678884577.7239003 [executor_node-8] (:requirements :typing :negative-preconditions :durative-actions)
1678884577.7239411 [executor_node-8] (:types
1678884577.7239749 [executor_node-8] 	door
1678884577.7240303 [executor_node-8] 	sound
1678884577.7240658 [executor_node-8] 	wp
1678884577.7240963 [executor_node-8] )
1678884577.7241285 [executor_node-8] (:predicates
1678884577.7241755 [executor_node-8] 	(door_at ?d0 - door ?w1 - wp)
1678884577.7242112 [executor_node-8] 	(door_checked ?d0 - door)
1678884577.7242436 [executor_node-8] 	(robot_at ?w0 - wp)
1678884577.7242765 [executor_node-8] 	(sound_listened ?s0 - sound)
1678884577.7243075 [executor_node-8] )
1678884577.7243369 [executor_node-8] (:durative-action check_door
1678884577.7243667 [executor_node-8] 	:parameters ( ?wp - wp ?door - door)
1678884577.7243962 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7244265 [executor_node-8] 	:condition (and
1678884577.7244639 [executor_node-8] 		(at start (door_at ?door ?wp))
1678884577.7245104 [executor_node-8] 		(at start (robot_at ?wp))
1678884577.7245495 [executor_node-8] 	)
1678884577.7245889 [executor_node-8] 	:effect (and
1678884577.7246275 [executor_node-8] 		(at end (door_checked ?door))
1678884577.7246664 [executor_node-8] 	)
1678884577.7247052 [executor_node-8] )
1678884577.7247431 [executor_node-8] (:durative-action navigation
1678884577.7247810 [executor_node-8] 	:parameters ( ?o - wp ?d - wp)
1678884577.7248192 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7248578 [executor_node-8] 	:condition (and
1678884577.7248914 [executor_node-8] 		(at start (robot_at ?o))
1678884577.7249236 [executor_node-8] 	)
1678884577.7249556 [executor_node-8] 	:effect (and
1678884577.7249880 [executor_node-8] 		(at end (robot_at ?d))
1678884577.7250199 [executor_node-8] 		(at start (not (robot_at ?o)))
1678884577.7250516 [executor_node-8] 	)
1678884577.7250829 [executor_node-8] )
1678884577.7251143 [executor_node-8] )
1678884577.7251461 [executor_node-8] 
1678884577.7254245 [executor_node-8] [INFO] [1678884577.723845161] [merlin2.executor_node]: (define (problem merlin2_prb)
1678884577.7254870 [executor_node-8] (:domain merlin2)
1678884577.7255244 [executor_node-8] (:objects
1678884577.7255585 [executor_node-8] 	boiling - sound
1678884577.7255921 [executor_node-8] 	door_entrance - door
1678884577.7256258 [executor_node-8] 	doorbell - sound
1678884577.7256558 [executor_node-8] 	entrance - wp
1678884577.7256918 [executor_node-8] 	insect - sound
1678884577.7257254 [executor_node-8] 	inside_small_room - sound
1678884577.7257576 [executor_node-8] 	livingroom - wp
1678884577.7257905 [executor_node-8] 	mechanical_fan - sound
1678884577.7258232 [executor_node-8] 	music - sound
1678884577.7258549 [executor_node-8] 	rustle - sound
1678884577.7258875 [executor_node-8] 	tubular_bells - sound
1678884577.7259202 [executor_node-8] 	white_noise - sound
1678884577.7259526 [executor_node-8] )
1678884577.7259843 [executor_node-8] (:init
1678884577.7260165 [executor_node-8] 	(robot_at livingroom)
1678884577.7260485 [executor_node-8] 	(door_at door_entrance entrance)
1678884577.7260811 [executor_node-8] 	(sound_listened tubular_bells)
1678884577.7261131 [executor_node-8] )
1678884577.7261448 [executor_node-8] (:goal
1678884577.7261763 [executor_node-8] 	(and
1678884577.7262082 [executor_node-8] 	(door_checked door_entrance)
1678884577.7262411 [executor_node-8] 	(robot_at livingroom)
1678884577.7262723 [executor_node-8] 	)
1678884577.7263045 [executor_node-8] )
1678884577.7263389 [executor_node-8] )
1678884577.7263732 [executor_node-8] 
1678884577.7265377 [planner_node-6] [INFO] [1678884577.725191561] [merlin2.planner_node]: Plan is resolved with: UPF planner
1678884577.7749512 [planner_node-6] [INFO] [1678884577.774736152] [merlin2.planner_node]: problem name = merlin2_prb
1678884577.7750733 [planner_node-6] 
1678884577.7751172 [planner_node-6] types = [door, sound, wp]
1678884577.7751536 [planner_node-6] 
1678884577.7751887 [planner_node-6] fluents = [
1678884577.7752166 [planner_node-6]   bool door_at[d0=door, w1=wp]
1678884577.7752433 [planner_node-6]   bool door_checked[d0=door]
1678884577.7752690 [planner_node-6]   bool robot_at[w0=wp]
1678884577.7752948 [planner_node-6]   bool sound_listened[s0=sound]
1678884577.7753203 [planner_node-6] ]
1678884577.7753584 [planner_node-6] 
1678884577.7753849 [planner_node-6] actions = [
1678884577.7754109 [planner_node-6]   durative action check_door(wp wp, door door) {
1678884577.7754376 [planner_node-6]     duration = [10, 10]
1678884577.7754636 [planner_node-6]     conditions = [
1678884577.7754891 [planner_node-6]       [start]:
1678884577.7755139 [planner_node-6]         door_at(door, wp)
1678884577.7755392 [planner_node-6]         robot_at(wp)
1678884577.7755644 [planner_node-6]     ]
1678884577.7755895 [planner_node-6]     effects = [
1678884577.7756147 [planner_node-6]       end:
1678884577.7756398 [planner_node-6]         door_checked(door) := true:
1678884577.7756650 [planner_node-6]     ]
1678884577.7756970 [planner_node-6]     simulated effects = [
1678884577.7757330 [planner_node-6]     ]
1678884577.7757671 [planner_node-6]   }
1678884577.7758024 [planner_node-6]   durative action navigation(wp o, wp d) {
1678884577.7758374 [planner_node-6]     duration = [10, 10]
1678884577.7758744 [planner_node-6]     conditions = [
1678884577.7759106 [planner_node-6]       [start]:
1678884577.7759442 [planner_node-6]         robot_at(o)
1678884577.7759795 [planner_node-6]     ]
1678884577.7760427 [planner_node-6]     effects = [
1678884577.7761126 [planner_node-6]       end:
1678884577.7761495 [planner_node-6]         robot_at(d) := true:
1678884577.7761836 [planner_node-6]       start:
1678884577.7762163 [planner_node-6]         robot_at(o) := false:
1678884577.7762508 [planner_node-6]     ]
1678884577.7762845 [planner_node-6]     simulated effects = [
1678884577.7763171 [planner_node-6]     ]
1678884577.7763495 [planner_node-6]   }
1678884577.7763817 [planner_node-6] ]
1678884577.7764144 [planner_node-6] 
1678884577.7765701 [planner_node-6] objects = [
1678884577.7766209 [planner_node-6]   door: [door_entrance]
1678884577.7766600 [planner_node-6]   sound: [boiling, doorbell, insect, inside_small_room, mechanical_fan, music, rustle, tubular_bells, white_noise]
1678884577.7766962 [planner_node-6]   wp: [entrance, livingroom]
1678884577.7767313 [planner_node-6] ]
1678884577.7767661 [planner_node-6] 
1678884577.7768130 [planner_node-6] initial fluents default = [
1678884577.7768567 [planner_node-6]   bool door_at[d0=door, w1=wp] := false
1678884577.7768998 [planner_node-6]   bool door_checked[d0=door] := false
1678884577.7769418 [planner_node-6]   bool robot_at[w0=wp] := false
1678884577.7769835 [planner_node-6]   bool sound_listened[s0=sound] := false
1678884577.7770252 [planner_node-6] ]
1678884577.7770660 [planner_node-6] 
1678884577.7771068 [planner_node-6] initial values = [
1678884577.7771471 [planner_node-6]   robot_at(livingroom) := true
1678884577.7771890 [planner_node-6]   door_at(door_entrance, entrance) := true
1678884577.7772298 [planner_node-6]   sound_listened(tubular_bells) := true
1678884577.7772694 [planner_node-6] ]
1678884577.7773125 [planner_node-6] 
1678884577.7773521 [planner_node-6] goals = [
1678884577.7773938 [planner_node-6]   (door_checked(door_entrance) and robot_at(livingroom))
1678884577.7774792 [planner_node-6] ]
1678884577.7775264 [planner_node-6] 
1678884577.7775741 [planner_node-6] 
1678884577.7780237 [planner_node-6] [INFO] [1678884577.775027739] [merlin2.planner_node]: [(Fraction(0, 1), navigation(livingroom, entrance), Fraction(10, 1)), (Fraction(1001, 100), check_door(entrance, door_entrance), Fraction(10, 1)), (Fraction(1001, 100), navigation(entrance, livingroom), Fraction(10, 1))]
1678884577.7783008 [executor_node-8] [INFO] [1678884577.776828442] [merlin2.executor_node]: merlin2_arch_interfaces.srv.GeneratePlan_Response(plan=[merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])], has_solution=True)
1678884577.7783656 [executor_node-8] [INFO] [1678884577.777149872] [merlin2.executor_node]: Plan has solution: True
1678884577.7784219 [executor_node-8] [INFO] [1678884577.777416267] [merlin2.executor_node]: [merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])]
1678884577.8014164 [plan_dispatcher_node-7] [INFO] [1678884577.801176089] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['livingroom', 'entrance']
1678884578.7195942 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884578.7204616 [sound_recognition_node-2] [INFO] [1678884578.720231403] [sound_recognition.sound_recognition_node]: alarm_clock
1678884580.0046661 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884580.0055346 [sound_recognition_node-2] [INFO] [1678884580.005407062] [sound_recognition.sound_recognition_node]: bell
1678884580.0484161 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884580.0497820 [sound_recognition_node-2] [INFO] [1678884580.049492234] [sound_recognition.sound_recognition_node]: vehicle
1678884581.0828433 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884581.0841291 [sound_recognition_node-2] [INFO] [1678884581.083873352] [sound_recognition.sound_recognition_node]: music
1678884582.3525014 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884582.3536935 [sound_recognition_node-2] [INFO] [1678884582.353561880] [sound_recognition.sound_recognition_node]: music
1678884583.6463435 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884583.6471636 [sound_recognition_node-2] [INFO] [1678884583.647013382] [sound_recognition.sound_recognition_node]: vehicle
1678884584.7310882 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884584.7319632 [sound_recognition_node-2] [INFO] [1678884584.731796092] [sound_recognition.sound_recognition_node]: vehicle
1678884586.0069947 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884586.0082140 [sound_recognition_node-2] [INFO] [1678884586.008029948] [sound_recognition.sound_recognition_node]: car
1678884586.0511088 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884586.0525103 [sound_recognition_node-2] [INFO] [1678884586.052294635] [sound_recognition.sound_recognition_node]: music
1678884587.0782769 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884587.0792749 [sound_recognition_node-2] [INFO] [1678884587.079105365] [sound_recognition.sound_recognition_node]: music
1678884588.3589358 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884588.3597465 [sound_recognition_node-2] [INFO] [1678884588.359540684] [sound_recognition.sound_recognition_node]: fire
1678884589.6029940 [plan_dispatcher_node-7] [INFO] [1678884589.602774557] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884589.6080005 [plan_dispatcher_node-7] [INFO] [1678884589.607784180] [merlin2.plan_dispatcher_node]: Executing action check_door with objects ['entrance', 'door_entrance']
1678884589.6557701 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884589.6566753 [sound_recognition_node-2] [INFO] [1678884589.656506238] [sound_recognition.sound_recognition_node]: vehicle
1678884590.7275991 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884590.7283554 [sound_recognition_node-2] [INFO] [1678884590.728173845] [sound_recognition.sound_recognition_node]: vehicle
1678884592.0076108 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0087211 [sound_recognition_node-2] [INFO] [1678884592.008428457] [sound_recognition.sound_recognition_node]: cat
1678884592.0485382 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0494387 [sound_recognition_node-2] [INFO] [1678884592.049249248] [sound_recognition.sound_recognition_node]: purr
1678884593.0732682 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884593.0742242 [sound_recognition_node-2] [INFO] [1678884593.074061453] [sound_recognition.sound_recognition_node]: purr
1678884594.3611791 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884594.3619897 [sound_recognition_node-2] [INFO] [1678884594.361858576] [sound_recognition.sound_recognition_node]: purr
1678884595.6587839 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884595.6597569 [sound_recognition_node-2] [INFO] [1678884595.659593389] [sound_recognition.sound_recognition_node]: purr
1678884596.7353518 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884596.7362726 [sound_recognition_node-2] [INFO] [1678884596.736126401] [sound_recognition.sound_recognition_node]: aircraft
1678884598.0120232 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884598.0135968 [sound_recognition_node-2] [INFO] [1678884598.013389874] [sound_recognition.sound_recognition_node]: vehicle
1678884598.0607984 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 24ms/step
1678884598.0616784 [sound_recognition_node-2] [INFO] [1678884598.061512502] [sound_recognition.sound_recognition_node]: white_noise
1678884598.7223277 [plan_dispatcher_node-7] [INFO] [1678884598.721810188] [merlin2.plan_dispatcher_node]: Action check_door finished
1678884598.7302756 [plan_dispatcher_node-7] [INFO] [1678884598.729979771] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['entrance', 'livingroom']
1678884599.0797648 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884599.0813777 [sound_recognition_node-2] [INFO] [1678884599.081100644] [sound_recognition.sound_recognition_node]: cat
1678884600.3607635 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884600.3616989 [sound_recognition_node-2] [INFO] [1678884600.361469893] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884601.6549842 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884601.6558256 [sound_recognition_node-2] [INFO] [1678884601.655628147] [sound_recognition.sound_recognition_node]: vehicle
1678884602.7287250 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884602.7296121 [sound_recognition_node-2] [INFO] [1678884602.729406425] [sound_recognition.sound_recognition_node]: fireworks
1678884604.0130072 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0138850 [sound_recognition_node-2] [INFO] [1678884604.013727869] [sound_recognition.sound_recognition_node]: vehicle
1678884604.0554757 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0564170 [sound_recognition_node-2] [INFO] [1678884604.056236505] [sound_recognition.sound_recognition_node]: vehicle
1678884605.0930657 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884605.0940287 [sound_recognition_node-2] [INFO] [1678884605.093870245] [sound_recognition.sound_recognition_node]: car
1678884606.3664958 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884606.3674438 [sound_recognition_node-2] [INFO] [1678884606.367253105] [sound_recognition.sound_recognition_node]: speech
1678884607.6561847 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884607.6574214 [sound_recognition_node-2] [INFO] [1678884607.657066928] [sound_recognition.sound_recognition_node]: vehicle
1678884608.7308884 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884608.7318692 [sound_recognition_node-2] [INFO] [1678884608.731702736] [sound_recognition.sound_recognition_node]: door
1678884610.0239010 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884610.0249777 [sound_recognition_node-2] [INFO] [1678884610.024740027] [sound_recognition.sound_recognition_node]: clip-clop
1678884610.0709939 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884610.0720925 [sound_recognition_node-2] [INFO] [1678884610.071893309] [sound_recognition.sound_recognition_node]: vehicle
1678884611.0926340 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884611.0935619 [sound_recognition_node-2] [INFO] [1678884611.093425957] [sound_recognition.sound_recognition_node]: run
1678884612.3709085 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 21ms/step
1678884612.3721375 [sound_recognition_node-2] [INFO] [1678884612.371996360] [sound_recognition.sound_recognition_node]: vehicle
1678884613.6597800 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884613.6606991 [sound_recognition_node-2] [INFO] [1678884613.660547206] [sound_recognition.sound_recognition_node]: fireworks
1678884614.6283243 [plan_dispatcher_node-7] [INFO] [1678884614.628098842] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884614.6424882 [executor_node-8] [INFO] [1678884614.642279934] [merlin2.executor_node]: Removing goals
1678884614.6521719 [merlin2_demo3_node-12] [INFO] [1678884614.651949485] [merlin2.merlin2_demo3_node]: results got
1678884614.6525984 [merlin2_demo3_node-12] [INFO] [1678884614.652343977] [merlin2.merlin2_demo3_node]: True
1678884614.6528592 [merlin2_demo3_node-12] [INFO] [1678884614.652701010] [merlin2.merlin2_demo3_node]: Execution time: 37.00015163421631
1678884614.7444584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884614.7458823 [sound_recognition_node-2] [INFO] [1678884614.745525474] [sound_recognition.sound_recognition_node]: vehicle
1678884615.3285997 [INFO] [merlin2_demo3_node-12]: process has finished cleanly [pid 116658]
1678884616.0222907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884616.0231855 [sound_recognition_node-2] [INFO] [1678884616.023015762] [sound_recognition.sound_recognition_node]: speech
1678884616.0596013 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884616.0607092 [sound_recognition_node-2] [INFO] [1678884616.060568587] [sound_recognition.sound_recognition_node]: animal
1678884617.0980983 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884617.0989578 [sound_recognition_node-2] [INFO] [1678884617.098742894] [sound_recognition.sound_recognition_node]: purr
1678884618.3806093 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884618.3815532 [sound_recognition_node-2] [INFO] [1678884618.381186176] [sound_recognition.sound_recognition_node]: cat
1678884619.6675181 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884619.6683767 [sound_recognition_node-2] [INFO] [1678884619.668243642] [sound_recognition.sound_recognition_node]: white_noise
1678884620.7404547 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884620.7412405 [sound_recognition_node-2] [INFO] [1678884620.741016751] [sound_recognition.sound_recognition_node]: cat
1678884622.0207660 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884622.0216982 [sound_recognition_node-2] [INFO] [1678884622.021457515] [sound_recognition.sound_recognition_node]: fireworks
1678884622.0633199 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884622.0647492 [sound_recognition_node-2] [INFO] [1678884622.064380576] [sound_recognition.sound_recognition_node]: fireworks
1678884623.1012793 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884623.1021008 [sound_recognition_node-2] [INFO] [1678884623.101955993] [sound_recognition.sound_recognition_node]: cat
1678884624.3767979 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884624.3777966 [sound_recognition_node-2] [INFO] [1678884624.377584603] [sound_recognition.sound_recognition_node]: cat
1678884625.6724491 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884625.6735289 [sound_recognition_node-2] [INFO] [1678884625.673325423] [sound_recognition.sound_recognition_node]: cat
1678884626.7613523 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884626.7623341 [sound_recognition_node-2] [INFO] [1678884626.762190369] [sound_recognition.sound_recognition_node]: fireworks
1678884628.0220890 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0229340 [sound_recognition_node-2] [INFO] [1678884628.022791220] [sound_recognition.sound_recognition_node]: animal
1678884628.0623763 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0631883 [sound_recognition_node-2] [INFO] [1678884628.063056020] [sound_recognition.sound_recognition_node]: animal
1678884629.1064036 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884629.1073856 [sound_recognition_node-2] [INFO] [1678884629.107205676] [sound_recognition.sound_recognition_node]: animal
1678884630.3849888 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884630.3859134 [sound_recognition_node-2] [INFO] [1678884630.385733439] [sound_recognition.sound_recognition_node]: cat
1678884631.6770473 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884631.6780236 [sound_recognition_node-2] [INFO] [1678884631.677869932] [sound_recognition.sound_recognition_node]: cat
1678884632.7579663 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884632.7588894 [sound_recognition_node-2] [INFO] [1678884632.758740682] [sound_recognition.sound_recognition_node]: speech
1678884634.0236197 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884634.0247653 [sound_recognition_node-2] [INFO] [1678884634.024479737] [sound_recognition.sound_recognition_node]: fireworks
1678884634.0605907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884634.0614641 [sound_recognition_node-2] [INFO] [1678884634.061317538] [sound_recognition.sound_recognition_node]: fireworks
1678884635.1101820 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884635.1112704 [sound_recognition_node-2] [INFO] [1678884635.111035945] [sound_recognition.sound_recognition_node]: vehicle
1678884636.3903909 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884636.3913989 [sound_recognition_node-2] [INFO] [1678884636.391185251] [sound_recognition.sound_recognition_node]: motorcycle
1678884637.6810584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884637.6820164 [sound_recognition_node-2] [INFO] [1678884637.681732562] [sound_recognition.sound_recognition_node]: stomach_rumble
1678884638.7616808 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884638.7624626 [sound_recognition_node-2] [INFO] [1678884638.762324844] [sound_recognition.sound_recognition_node]: computer_keyboard
1678884639.9263844 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT)
1678884639.9375060 [planner_node-6] [INFO] [1678884639.927608639] [merlin2.planner_node]: Destroying node planner_node
1678884639.9376597 [planner_node-6] Traceback (most recent call last):
1678884639.9377372 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 124, in <module>
1678884639.9378009 [planner_node-6]     main()
1678884639.9378636 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 118, in main
1678884639.9379246 [planner_node-6]     node.join_spin()
1678884639.9379847 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9380448 [planner_node-6]     self._spin_thread.join()
1678884639.9381051 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9381669 [planner_node-6]     self._wait_for_tstate_lock()
1678884639.9382248 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9382832 [planner_node-6]     if lock.acquire(block, timeout):
1678884639.9383414 [planner_node-6] KeyboardInterrupt
1678884639.9386270 [executor_node-8] [INFO] [1678884639.927741220] [merlin2.executor_node]: Destroying node executor_node
1678884639.9387064 [executor_node-8] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9388056 [executor_node-8] Traceback (most recent call last):
1678884639.9388685 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node", line 33, in <module>
1678884639.9389281 [executor_node-8]     sys.exit(load_entry_point('merlin2-executor==0.0.0', 'console_scripts', 'executor_node')())
1678884639.9389863 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/python3.10/site-packages/merlin2_executor/merlin2_executor_node.py", line 101, in main
1678884639.9390466 [executor_node-8]     node.join_spin()
1678884639.9391050 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9391639 [executor_node-8]     self._spin_thread.join()
1678884639.9392228 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9392829 [executor_node-8]     self._wait_for_tstate_lock()
1678884639.9393370 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9393902 [executor_node-8]     if lock.acquire(block, timeout):
1678884639.9394498 [executor_node-8] KeyboardInterrupt
1678884639.9397473 [planner_node-6] [96m[1mNOTE: To disable printing of planning engine credits, add this line to your code: `up.shortcuts.get_environment().credits_stream = None`
1678884639.9397938 [planner_node-6] [0m[96m  *** Credits ***
1678884639.9398353 [planner_node-6] [0m[96m  * In operation mode `OneshotPlanner` at line 72 of `/home/gentlebots/ros2_ws/install/merlin2_planner/local/lib/python3.10/dist-packages/merlin2_planner/merlin2_planners/up_merlin2_planner.py`, [0m[96myou are using the following planning engine:
1678884639.9398808 [planner_node-6] [0m[96m  * Engine name: Tamer
1678884639.9399147 [planner_node-6]   * Developers:  FBK Tamer Development Team
1678884639.9399474 [planner_node-6] [0m[96m  * Description: [0m[96mTamer offers the capability to generate a plan for classical, numerical and temporal problems.
1678884639.9399786 [planner_node-6]   *              For those kind of problems tamer also offers the possibility of validating a submitted plan.[0m[96m
1678884639.9400105 [planner_node-6] [0m[96m
1678884639.9402139 [merlin2_listen_audio_node-9] Traceback (most recent call last):
1678884639.9402971 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node", line 33, in <module>
1678884639.9403560 [merlin2_listen_audio_node-9]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_listen_audio_node')())
1678884639.9404116 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_listen_audio_node.py", line 60, in main
1678884639.9404681 [merlin2_listen_audio_node-9]     rclpy.spin(node_listen)
1678884639.9405236 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9405794 [merlin2_listen_audio_node-9]     executor.spin_once()
1678884639.9406352 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9406912 [merlin2_listen_audio_node-9]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9407454 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9407988 [merlin2_listen_audio_node-9]     return next(self._cb_iter)
1678884639.9408545 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9409101 [merlin2_listen_audio_node-9]     wait_set.wait(timeout_nsec)
1678884639.9409649 [merlin2_listen_audio_node-9] KeyboardInterrupt
1678884639.9412544 [sound_recognition_node-2] Traceback (most recent call last):
1678884639.9413280 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node", line 33, in <module>
1678884639.9413857 [sound_recognition_node-2]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'sound_recognition_node')())
1678884639.9414403 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/sound_recognition_node.py", line 180, in main
1678884639.9414942 [sound_recognition_node-2]     rclpy.spin(sound_recognition_node)
1678884639.9415493 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9416041 [sound_recognition_node-2]     executor.spin_once()
1678884639.9416573 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9417100 [sound_recognition_node-2]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9417644 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9418187 [sound_recognition_node-2]     return next(self._cb_iter)
1678884639.9418733 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9419284 [sound_recognition_node-2]     wait_set.wait(timeout_nsec)
1678884639.9419937 [sound_recognition_node-2] KeyboardInterrupt
1678884639.9422145 [plan_dispatcher_node-7] [INFO] [1678884639.935175976] [merlin2.plan_dispatcher_node]: Destroying node plan_dispatcher_node
1678884639.9422836 [plan_dispatcher_node-7] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9699667 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884639.9701345 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 261, in <module>
1678884639.9705858 [plan_dispatcher_node-7]     main()
1678884639.9707761 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 255, in main
1678884639.9708421 [plan_dispatcher_node-7]     node.join_spin()
1678884639.9708920 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9709430 [plan_dispatcher_node-7]     self._spin_thread.join()
1678884639.9709916 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9710422 [plan_dispatcher_node-7]     self._wait_for_tstate_lock()
1678884639.9710903 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9714367 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884639.9715178 [plan_dispatcher_node-7] KeyboardInterrupt
1678884639.9827285 [waypoint_navigation_node-1] [INFO] [1678884639.982360745] [waypoint_navigation.waypoint_navigation_node]: Destroying node waypoint_navigation_node
1678884639.9828951 [waypoint_navigation_node-1] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0044258 [tts_node-4] [INFO] [1678884640.004114039] [text_to_speech.tts_node]: Destroying node tts_node
1678884640.0055861 [tts_node-4] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0089176 [pddl_generator_node-5] [INFO] [1678884640.008586743] [merlin2.pddl_generator_node]: Destroying node pddl_generator_node
1678884640.0110254 [pddl_generator_node-5] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0383022 [tts_node-4] Traceback (most recent call last):
1678884640.0384836 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node", line 33, in <module>
1678884640.0392134 [tts_node-4]     sys.exit(load_entry_point('text-to-speech==0.0.0', 'console_scripts', 'tts_node')())
1678884640.0393784 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/python3.10/site-packages/text_to_speech/tts_node.py", line 88, in main
1678884640.0398426 [tts_node-4]     node.join_spin()
1678884640.0404348 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0405629 [tts_node-4]     self._spin_thread.join()
1678884640.0406227 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0408790 [tts_node-4]     self._wait_for_tstate_lock()
1678884640.0409479 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0414391 [tts_node-4]     if lock.acquire(block, timeout):
1678884640.0415742 [tts_node-4] KeyboardInterrupt
1678884640.0486207 [manager_node-3] [INFO] [1678884640.048209927] [sound_recognition.manager_node]: Destroying node manager_node
1678884640.0491898 [manager_node-3] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0594249 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.0598230 [executor_node-8] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0599537 [executor_node-8] Traceback (most recent call last):
1678884640.0600307 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0600920 [executor_node-8]     lock.acquire()
1678884640.0601518 [executor_node-8] KeyboardInterrupt: 
1678884640.0606339 [plan_dispatcher_node-7] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f13a644d120>
1678884640.0607460 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884640.0608060 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.0608621 [plan_dispatcher_node-7]     shutdown()
1678884640.0609159 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.0609689 [plan_dispatcher_node-7]     executor.join(1)
1678884640.0610261 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.0610845 [plan_dispatcher_node-7]     self._thread.join(timeout)
1678884640.0611324 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.0614121 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0615094 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0615876 [merlin2_navigation_fsm_action-10]     self._spin_thread.join()
1678884640.0616488 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0617082 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock()
1678884640.0617681 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0621009 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0621994 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0622642 [merlin2_check_door_fsm_action-11]     self._spin_thread.join()
1678884640.0623169 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0626640 [plan_dispatcher_node-7]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.0627830 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0628428 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884640.0628955 [plan_dispatcher_node-7] KeyboardInterrupt: 
1678884640.0631788 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.0632725 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0633259 [merlin2_navigation_fsm_action-10] 
1678884640.0633750 [merlin2_navigation_fsm_action-10] During handling of the above exception, another exception occurred:
1678884640.0634604 [merlin2_navigation_fsm_action-10] 
1678884640.0635068 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0635514 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action", line 33, in <module>
1678884640.0635984 [merlin2_navigation_fsm_action-10]     sys.exit(load_entry_point('merlin2-basic-actions==0.0.0', 'console_scripts', 'merlin2_navigation_fsm_action')())
1678884640.0636446 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/python3.10/site-packages/merlin2_basic_actions/merlin2_navigation_fsm_action.py", line 79, in main
1678884640.0637033 [merlin2_navigation_fsm_action-10]     node.join_spin()
1678884640.0637522 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0638134 [merlin2_navigation_fsm_action-10]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0638635 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0642893 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock()
1678884640.0643778 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0644319 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.0645759 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0646703 [merlin2_check_door_fsm_action-11] 
1678884640.0647247 [merlin2_check_door_fsm_action-11] During handling of the above exception, another exception occurred:
1678884640.0647728 [merlin2_check_door_fsm_action-11] 
1678884640.0648203 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0648930 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action", line 33, in <module>
1678884640.0657759 [merlin2_check_door_fsm_action-11]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_check_door_fsm_action')())
1678884640.0658810 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_check_door_fsm_action.py", line 113, in main
1678884640.0659249 [merlin2_check_door_fsm_action-11]     node.join_spin()
1678884640.0659778 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0660744 [merlin2_check_door_fsm_action-11]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0661254 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0661690 [merlin2_check_door_fsm_action-11]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0662074 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0662374 [merlin2_check_door_fsm_action-11]     caller_id = CallerId()
1678884640.0662651 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0662911 [merlin2_check_door_fsm_action-11]     frame = _find_caller(inspect.currentframe())
1678884640.0663180 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0663452 [merlin2_check_door_fsm_action-11]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0663724 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0665815 [ERROR] [tts_node-4]: process has died [pid 116642, exit code -2, cmd '/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node --ros-args -r __node:=tts_node -r __ns:=/text_to_speech'].
1678884640.0668547 [ERROR] [planner_node-6]: process has died [pid 116646, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node --ros-args -r __node:=planner_node --params-file /tmp/launch_params_7r3e82of'].
1678884640.0670576 [merlin2_navigation_fsm_action-10]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0671303 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0671668 [merlin2_navigation_fsm_action-10]     caller_id = CallerId()
1678884640.0671957 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0672326 [merlin2_navigation_fsm_action-10]     frame = _find_caller(inspect.currentframe())
1678884640.0672596 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0672865 [merlin2_navigation_fsm_action-10]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0673132 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0674167 [ERROR] [merlin2_listen_audio_node-9]: process has died [pid 116652, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node --ros-args -r __node:=listen_audio_node --params-file /tmp/launch_params_2cv5d0ur'].
1678884640.0676262 [sound_recognition_node-2] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0676715 [sound_recognition_node-2] Traceback (most recent call last):
1678884640.0677016 [sound_recognition_node-2]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0677290 [sound_recognition_node-2]     lock.acquire()
1678884640.0677621 [sound_recognition_node-2] KeyboardInterrupt: 
1678884640.0682333 [planner_node-6] [0m
1678884640.0684013 [merlin2_check_door_fsm_action-11]     lines, lnum = findsource(frame)
1678884640.0684705 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0685141 [merlin2_check_door_fsm_action-11]     module = getmodule(object, file)
1678884640.0685487 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0685754 [merlin2_check_door_fsm_action-11]     os.path.realpath(f)] = module.__name__
1678884640.0686009 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 395, in realpath
1678884640.0686257 [merlin2_check_door_fsm_action-11]     path, ok = _joinrealpath(filename[:0], filename, strict, {})
1678884640.0686502 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 430, in _joinrealpath
1678884640.0686753 [merlin2_check_door_fsm_action-11]     st = os.lstat(newpath)
1678884640.0687015 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0688329 [merlin2_navigation_fsm_action-10]     lines, lnum = findsource(frame)
1678884640.0688710 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0688999 [merlin2_navigation_fsm_action-10]     module = getmodule(object, file)
1678884640.0689266 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0689526 [merlin2_navigation_fsm_action-10]     os.path.realpath(f)] = module.__name__
1678884640.0689790 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 396, in realpath
1678884640.0691872 [merlin2_navigation_fsm_action-10]     return abspath(path)
1678884640.0692399 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 385, in abspath
1678884640.0692704 [merlin2_navigation_fsm_action-10]     return normpath(path)
1678884640.0692973 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 370, in normpath
1678884640.0693257 [merlin2_navigation_fsm_action-10]     path = sep.join(comps)
1678884640.0693529 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0708385 [sound_recognition_node-2] terminate called without an active exception
1678884640.0950975 [ERROR] [sound_recognition_node-2]: process has died [pid 116638, exit code -6, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node --ros-args -r __node:=sound_recognition_node -r __ns:=/sound_recognition'].
1678884640.1990383 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.1997647 [merlin2_navigation_fsm_action-10] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.1999891 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.2001505 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2008882 [merlin2_check_door_fsm_action-11] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.2010698 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.2012010 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2017617 [merlin2_navigation_fsm_action-10]     lock.acquire()
1678884640.2019246 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.2024467 [merlin2_check_door_fsm_action-11]     lock.acquire()
1678884640.2026238 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.2085764 [ERROR] [executor_node-8]: process has died [pid 116650, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node --ros-args -r __node:=executor_node --params-file /tmp/launch_params_pm3nbifn'].
1678884640.2101398 [ERROR] [plan_dispatcher_node-7]: process has died [pid 116648, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node --ros-args -r __node:=plan_dispatcher_node --params-file /tmp/launch_params__aeqwv7a'].
1678884640.3144882 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.3149836 [merlin2_check_door_fsm_action-11] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f3a284ffac0>
1678884640.3151383 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.3152375 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3153253 [merlin2_check_door_fsm_action-11]     shutdown()
1678884640.3154082 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3154931 [merlin2_check_door_fsm_action-11]     executor.join(1)
1678884640.3155742 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3156583 [merlin2_check_door_fsm_action-11]     self._thread.join(timeout)
1678884640.3157396 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3162990 [merlin2_navigation_fsm_action-10] Exception ignored in atexit callback: <function _shutdown_resources at 0x7fe101593be0>
1678884640.3164382 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.3165314 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3166242 [merlin2_navigation_fsm_action-10]     shutdown()
1678884640.3167090 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3168330 [merlin2_navigation_fsm_action-10]     executor.join(1)
1678884640.3169751 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3171227 [merlin2_navigation_fsm_action-10]     self._thread.join(timeout)
1678884640.3172050 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3179805 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3181605 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3182542 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.3183537 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.3187332 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3188431 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3189273 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.3190041 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.4113688 [ERROR] [merlin2_check_door_fsm_action-11]: process has died [pid 116656, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action --ros-args -r __node:=check_door --params-file /tmp/launch_params_x5yoc90u'].
1678884640.4120762 [ERROR] [merlin2_navigation_fsm_action-10]: process has died [pid 116654, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action --ros-args -r __node:=navigation --params-file /tmp/launch_params_0i_ko1nb'].
1678884640.4295676 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.5633359 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.6955371 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884641.0691211 [manager_node-3] Traceback (most recent call last):
1678884641.0693920 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0700769 [manager_node-3]     self._spin_thread.join()
1678884641.0702577 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0704384 [manager_node-3]     self._wait_for_tstate_lock()
1678884641.0705881 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0712566 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0713716 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0718808 [waypoint_navigation_node-1]     self._spin_thread.join()
1678884641.0719829 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0721400 [waypoint_navigation_node-1]     self._wait_for_tstate_lock()
1678884641.0722322 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0722940 [waypoint_navigation_node-1]     if lock.acquire(block, timeout):
1678884641.0723536 [waypoint_navigation_node-1] KeyboardInterrupt
1678884641.0724115 [waypoint_navigation_node-1] 
1678884641.0724688 [waypoint_navigation_node-1] During handling of the above exception, another exception occurred:
1678884641.0725276 [waypoint_navigation_node-1] 
1678884641.0725942 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0726573 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node", line 33, in <module>
1678884641.0727687 [waypoint_navigation_node-1]     sys.exit(load_entry_point('waypoint-navigation==0.0.0', 'console_scripts', 'waypoint_navigation_node')())
1678884641.0729141 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/python3.10/site-packages/waypoint_navigation/waypoint_navigation_node.py", line 202, in main
1678884641.0734339 [waypoint_navigation_node-1]     node.join_spin()
1678884641.0735388 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0738482 [manager_node-3]     if lock.acquire(block, timeout):
1678884641.0739362 [manager_node-3] KeyboardInterrupt
1678884641.0740211 [manager_node-3] 
1678884641.0741096 [manager_node-3] During handling of the above exception, another exception occurred:
1678884641.0741870 [manager_node-3] 
1678884641.0742457 [manager_node-3] Traceback (most recent call last):
1678884641.0743215 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node", line 33, in <module>
1678884641.0743973 [manager_node-3]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'manager_node')())
1678884641.0744486 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/manager_node.py", line 111, in main
1678884641.0744917 [manager_node-3]     node.join_spin()
1678884641.0745425 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0746102 [manager_node-3]     self.destroy_node()
1678884641.0746596 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1683, in destroy_node
1678884641.0747027 [manager_node-3]     self.destroy_client(self._clients[0])
1678884641.0747452 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1593, in destroy_client
1678884641.0749857 [waypoint_navigation_node-1]     self.destroy_node()
1678884641.0750623 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884641.0753181 [waypoint_navigation_node-1]     self.destroy_service(self._services[0])
1678884641.0753920 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884641.0756521 [manager_node-3]     client.destroy()
1678884641.0758269 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/client.py", line 187, in destroy
1678884641.0761015 [manager_node-3]     self.__client.destroy_when_not_in_use()
1678884641.0761862 [manager_node-3] KeyboardInterrupt
1678884641.0764089 [waypoint_navigation_node-1]     service.destroy()
1678884641.0764818 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884641.0765414 [waypoint_navigation_node-1]     self.__service.destroy_when_not_in_use()
1678884641.0766015 [waypoint_navigation_node-1] KeyboardInterrupt
1678884642.1252923 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1256349 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884642.1265697 [pddl_generator_node-5]     self._spin_thread.join()
1678884642.1267729 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884642.1268961 [pddl_generator_node-5]     self._wait_for_tstate_lock()
1678884642.1270664 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884642.1277988 [pddl_generator_node-5]     if lock.acquire(block, timeout):
1678884642.1280391 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1282008 [pddl_generator_node-5] 
1678884642.1283841 [pddl_generator_node-5] During handling of the above exception, another exception occurred:
1678884642.1285546 [pddl_generator_node-5] 
1678884642.1286983 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1288023 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 63, in <module>
1678884642.1289310 [pddl_generator_node-5]     main()
1678884642.1290185 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 57, in main
1678884642.1294661 [pddl_generator_node-5]     node.join_spin()
1678884642.1296017 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884642.1300170 [pddl_generator_node-5]     self.destroy_node()
1678884642.1301351 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884642.1302304 [pddl_generator_node-5]     self.destroy_service(self._services[0])
1678884642.1302943 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884642.1306453 [pddl_generator_node-5]     service.destroy()
1678884642.1307805 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884642.1308813 [pddl_generator_node-5]     self.__service.destroy_when_not_in_use()
1678884642.1309750 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1558559 [ERROR] [manager_node-3]: process has died [pid 116640, exit code -2, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node --ros-args -r __node:=manager_node -r __ns:=/sound_recognition'].
1678884642.2004333 [ERROR] [waypoint_navigation_node-1]: process has died [pid 116636, exit code -2, cmd '/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node --ros-args -r __node:=waypoint_navigation_node -r __ns:=/waypoint_navigation --params-file /home/gentlebots/ros2_ws/install/waypoint_navigation/share/waypoint_navigation/params/apartamento_leon.yaml --params-file /tmp/launch_params_ret5a405'].
1678884642.6889017 [ERROR] [pddl_generator_node-5]: process has died [pid 116644, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node --ros-args -r __node:=pddl_generator_node --params-file /tmp/launch_params_l908797v'].


==> assets/launch_log_complete.tex <==

\begin{tiny}

\begin{Verbatim}[breaklines=true, breakanywhere=true]
1678884557.6391342 [INFO] [launch]: All log files can be found below /home/gentlebots/.ros/log/2023-03-15-13-49-17-632183-gentlebots-116634
1678884557.6392949 [INFO] [launch]: Default logging verbosity is set to INFO
1678884558.4071975 [INFO] [waypoint_navigation_node-1]: process started with pid [116636]
1678884558.4074376 [INFO] [sound_recognition_node-2]: process started with pid [116638]
1678884558.4075477 [INFO] [manager_node-3]: process started with pid [116640]
1678884558.4076343 [INFO] [tts_node-4]: process started with pid [116642]
1678884558.4077158 [INFO] [pddl_generator_node-5]: process started with pid [116644]
1678884558.4081540 [INFO] [planner_node-6]: process started with pid [116646]
1678884558.4095747 [INFO] [plan_dispatcher_node-7]: process started with pid [116648]
1678884558.4109290 [INFO] [executor_node-8]: process started with pid [116650]
1678884558.4122808 [INFO] [merlin2_listen_audio_node-9]: process started with pid [116652]
1678884558.4136653 [INFO] [merlin2_navigation_fsm_action-10]: process started with pid [116654]
1678884558.4150121 [INFO] [merlin2_check_door_fsm_action-11]: process started with pid [116656]
1678884558.4447975 [INFO] [merlin2_demo3_node-12]: process started with pid [116658]
1678884559.4909811 [tts_node-4] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6102691 [merlin2_check_door_fsm_action-11] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6540756 [planner_node-6] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.8783755 [manager_node-3] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.1545579 [waypoint_navigation_node-1] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3826396 [executor_node-8] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3833480 [pddl_generator_node-5] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.4762170 [waypoint_navigation_node-1] /opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py:441: UserWarning: when declaring parameter named 'wps', declaring a parameter only providing its name is deprecated. You have to either:
1678884560.4764743 [waypoint_navigation_node-1] 	- Pass a name and a default value different to "PARAMETER NOT SET" (and optionally a descriptor).
1678884560.4766202 [waypoint_navigation_node-1] 	- Pass a name and a parameter type.
1678884560.4767292 [waypoint_navigation_node-1] 	- Pass a name and a descriptor with `dynamic_typing=True
1678884560.4768608 [waypoint_navigation_node-1]   warnings.warn(
1678884560.4823425 [merlin2_demo3_node-12] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.5726750 [plan_dispatcher_node-7] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6693683 [merlin2_listen_audio_node-9] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6927030 [merlin2_navigation_fsm_action-10] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884561.2024031 [merlin2_demo3_node-12] [INFO] [1678884561.202155833] [merlin2.merlin2_demo3_node]: Waiting for doorbell...
1678884561.2941566 [sound_recognition_node-2] 2023-03-15 13:49:21.293771: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884561.2943850 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884561.5250556 [sound_recognition_node-2] 2023-03-15 13:49:21.524792: I tensorflow/core/util/port.cc:104] oneDNN custom operations are on. You may see slightly different numerical results due to floating-point round-off errors from different computation orders. To turn them off, set the environment variable `TF_ENABLE_ONEDNN_OPTS=0`.
1678884561.5278707 [sound_recognition_node-2] 2023-03-15 13:49:21.527592: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcudart.so.11.0'; dlerror: libcudart.so.11.0: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884561.5280049 [sound_recognition_node-2] 2023-03-15 13:49:21.527611: I tensorflow/compiler/xla/stream_executor/cuda/cudart_stub.cc:29] Ignore above cudart dlerror if you do not have a GPU set up on your machine.
1678884562.4255106 [sound_recognition_node-2] 2023-03-15 13:49:22.425286: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer.so.7'; dlerror: libnvinfer.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4259348 [sound_recognition_node-2] 2023-03-15 13:49:22.425422: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer_plugin.so.7'; dlerror: libnvinfer_plugin.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4260798 [sound_recognition_node-2] 2023-03-15 13:49:22.425431: W tensorflow/compiler/tf2tensorrt/utils/py_utils.cc:38] TF-TRT Warning: Cannot dlopen some TensorRT libraries. If you would like to use Nvidia GPU with TensorRT, please make sure the missing libraries mentioned above are installed properly.
1678884563.2107456 [sound_recognition_node-2] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884563.3666165 [sound_recognition_node-2] 2023-03-15 13:49:23.366304: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcuda.so.1'; dlerror: libcuda.so.1: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884563.3667796 [sound_recognition_node-2] 2023-03-15 13:49:23.366321: W tensorflow/compiler/xla/stream_executor/cuda/cuda_driver.cc:265] failed call to cuInit: UNKNOWN ERROR (303)
1678884563.3668425 [sound_recognition_node-2] 2023-03-15 13:49:23.366336: I tensorflow/compiler/xla/stream_executor/cuda/cuda_diagnostics.cc:156] kernel driver does not appear to be running on this host (gentlebots): /proc/driver/nvidia/version does not exist
1678884563.3672061 [sound_recognition_node-2] 2023-03-15 13:49:23.366532: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884563.3672807 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884564.7082698 [sound_recognition_node-2] [INFO] [1678884564.708041692] [sound_recognition.sound_recognition_node]: listen_thread starts listening
1678884564.7307980 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.front
1678884564.7310190 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.rear
1678884564.7310867 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.center_lfe
1678884564.7311323 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.side
1678884564.7312636 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313192 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313838 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround40
1678884564.7314229 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround41
1678884564.7318101 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround50
1678884564.7319388 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround51
1678884564.7319987 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround71
1678884564.7320669 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321129 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321570 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321966 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322392 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322824 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323217 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323618 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7326291 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7371376 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7373369 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7408085 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7409520 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7410004 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7410374 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7413969 [sound_recognition_node-2] ALSA lib pcm_dmix.c:1032:(snd_pcm_dmix_open) unable to open slave
1678884566.9160802 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 1s 841ms/step
1678884566.9175122 [sound_recognition_node-2] [INFO] [1678884566.917240165] [sound_recognition.sound_recognition_node]: music
1678884567.9730656 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884567.9741521 [sound_recognition_node-2] [INFO] [1678884567.973858829] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884568.0223629 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884568.0231643 [sound_recognition_node-2] [INFO] [1678884568.023020035] [sound_recognition.sound_recognition_node]: insect
1678884569.0709331 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884569.0717046 [sound_recognition_node-2] [INFO] [1678884569.071502259] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884570.3489144 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884570.3496821 [sound_recognition_node-2] [INFO] [1678884570.349498574] [sound_recognition.sound_recognition_node]: boiling
1678884571.6400306 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884571.6410005 [sound_recognition_node-2] [INFO] [1678884571.640862477] [sound_recognition.sound_recognition_node]: white_noise
1678884572.7147002 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884572.7157867 [sound_recognition_node-2] [INFO] [1678884572.715541398] [sound_recognition.sound_recognition_node]: rustle
1678884573.9964857 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884573.9973874 [sound_recognition_node-2] [INFO] [1678884573.997236108] [sound_recognition.sound_recognition_node]: inside_small_room
1678884574.0422242 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884574.0431235 [sound_recognition_node-2] [INFO] [1678884574.042970121] [sound_recognition.sound_recognition_node]: white_noise
1678884575.0656774 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884575.0665801 [sound_recognition_node-2] [INFO] [1678884575.066414965] [sound_recognition.sound_recognition_node]: white_noise
1678884576.3594229 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884576.3607428 [sound_recognition_node-2] [INFO] [1678884576.360408696] [sound_recognition.sound_recognition_node]: inside_small_room
1678884577.6447077 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884577.6457713 [sound_recognition_node-2] [INFO] [1678884577.645569064] [sound_recognition.sound_recognition_node]: tubular_bells
1678884577.6519880 [merlin2_demo3_node-12] [INFO] [1678884577.651800678] [merlin2.merlin2_demo3_node]: EXECUTING MISSION: Answer the door
1678884577.6523142 [merlin2_demo3_node-12] [INFO] [1678884577.652082970] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6556804 [merlin2_demo3_node-12] [INFO] [1678884577.655544354] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6559033 [merlin2_demo3_node-12] [INFO] [1678884577.655777629] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6604662 [merlin2_demo3_node-12] [INFO] [1678884577.660297157] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6607640 [merlin2_demo3_node-12] [INFO] [1678884577.660550771] [merlin2.merlin2_demo3_node]: goals saved
1678884577.6615767 [merlin2_demo3_node-12] [INFO] [1678884577.661483619] [merlin2.merlin2_demo3_node]: wait for results
1678884577.7237854 [executor_node-8] [INFO] [1678884577.723554341] [merlin2.executor_node]: (define (domain merlin2)
1678884577.7239003 [executor_node-8] (:requirements :typing :negative-preconditions :durative-actions)
1678884577.7239411 [executor_node-8] (:types
1678884577.7239749 [executor_node-8] 	door
1678884577.7240303 [executor_node-8] 	sound
1678884577.7240658 [executor_node-8] 	wp
1678884577.7240963 [executor_node-8] )
1678884577.7241285 [executor_node-8] (:predicates
1678884577.7241755 [executor_node-8] 	(door_at ?d0 - door ?w1 - wp)
1678884577.7242112 [executor_node-8] 	(door_checked ?d0 - door)
1678884577.7242436 [executor_node-8] 	(robot_at ?w0 - wp)
1678884577.7242765 [executor_node-8] 	(sound_listened ?s0 - sound)
1678884577.7243075 [executor_node-8] )
1678884577.7243369 [executor_node-8] (:durative-action check_door
1678884577.7243667 [executor_node-8] 	:parameters ( ?wp - wp ?door - door)
1678884577.7243962 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7244265 [executor_node-8] 	:condition (and
1678884577.7244639 [executor_node-8] 		(at start (door_at ?door ?wp))
1678884577.7245104 [executor_node-8] 		(at start (robot_at ?wp))
1678884577.7245495 [executor_node-8] 	)
1678884577.7245889 [executor_node-8] 	:effect (and
1678884577.7246275 [executor_node-8] 		(at end (door_checked ?door))
1678884577.7246664 [executor_node-8] 	)
1678884577.7247052 [executor_node-8] )
1678884577.7247431 [executor_node-8] (:durative-action navigation
1678884577.7247810 [executor_node-8] 	:parameters ( ?o - wp ?d - wp)
1678884577.7248192 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7248578 [executor_node-8] 	:condition (and
1678884577.7248914 [executor_node-8] 		(at start (robot_at ?o))
1678884577.7249236 [executor_node-8] 	)
1678884577.7249556 [executor_node-8] 	:effect (and
1678884577.7249880 [executor_node-8] 		(at end (robot_at ?d))
1678884577.7250199 [executor_node-8] 		(at start (not (robot_at ?o)))
1678884577.7250516 [executor_node-8] 	)
1678884577.7250829 [executor_node-8] )
1678884577.7251143 [executor_node-8] )
1678884577.7251461 [executor_node-8] 
1678884577.7254245 [executor_node-8] [INFO] [1678884577.723845161] [merlin2.executor_node]: (define (problem merlin2_prb)
1678884577.7254870 [executor_node-8] (:domain merlin2)
1678884577.7255244 [executor_node-8] (:objects
1678884577.7255585 [executor_node-8] 	boiling - sound
1678884577.7255921 [executor_node-8] 	door_entrance - door
1678884577.7256258 [executor_node-8] 	doorbell - sound
1678884577.7256558 [executor_node-8] 	entrance - wp
1678884577.7256918 [executor_node-8] 	insect - sound
1678884577.7257254 [executor_node-8] 	inside_small_room - sound
1678884577.7257576 [executor_node-8] 	livingroom - wp
1678884577.7257905 [executor_node-8] 	mechanical_fan - sound
1678884577.7258232 [executor_node-8] 	music - sound
1678884577.7258549 [executor_node-8] 	rustle - sound
1678884577.7258875 [executor_node-8] 	tubular_bells - sound
1678884577.7259202 [executor_node-8] 	white_noise - sound
1678884577.7259526 [executor_node-8] )
1678884577.7259843 [executor_node-8] (:init
1678884577.7260165 [executor_node-8] 	(robot_at livingroom)
1678884577.7260485 [executor_node-8] 	(door_at door_entrance entrance)
1678884577.7260811 [executor_node-8] 	(sound_listened tubular_bells)
1678884577.7261131 [executor_node-8] )
1678884577.7261448 [executor_node-8] (:goal
1678884577.7261763 [executor_node-8] 	(and
1678884577.7262082 [executor_node-8] 	(door_checked door_entrance)
1678884577.7262411 [executor_node-8] 	(robot_at livingroom)
1678884577.7262723 [executor_node-8] 	)
1678884577.7263045 [executor_node-8] )
1678884577.7263389 [executor_node-8] )
1678884577.7263732 [executor_node-8] 
1678884577.7265377 [planner_node-6] [INFO] [1678884577.725191561] [merlin2.planner_node]: Plan is resolved with: UPF planner
1678884577.7749512 [planner_node-6] [INFO] [1678884577.774736152] [merlin2.planner_node]: problem name = merlin2_prb
1678884577.7750733 [planner_node-6] 
1678884577.7751172 [planner_node-6] types = [door, sound, wp]
1678884577.7751536 [planner_node-6] 
1678884577.7751887 [planner_node-6] fluents = [
1678884577.7752166 [planner_node-6]   bool door_at[d0=door, w1=wp]
1678884577.7752433 [planner_node-6]   bool door_checked[d0=door]
1678884577.7752690 [planner_node-6]   bool robot_at[w0=wp]
1678884577.7752948 [planner_node-6]   bool sound_listened[s0=sound]
1678884577.7753203 [planner_node-6] ]
1678884577.7753584 [planner_node-6] 
1678884577.7753849 [planner_node-6] actions = [
1678884577.7754109 [planner_node-6]   durative action check_door(wp wp, door door) {
1678884577.7754376 [planner_node-6]     duration = [10, 10]
1678884577.7754636 [planner_node-6]     conditions = [
1678884577.7754891 [planner_node-6]       [start]:
1678884577.7755139 [planner_node-6]         door_at(door, wp)
1678884577.7755392 [planner_node-6]         robot_at(wp)
1678884577.7755644 [planner_node-6]     ]
1678884577.7755895 [planner_node-6]     effects = [
1678884577.7756147 [planner_node-6]       end:
1678884577.7756398 [planner_node-6]         door_checked(door) := true:
1678884577.7756650 [planner_node-6]     ]
1678884577.7756970 [planner_node-6]     simulated effects = [
1678884577.7757330 [planner_node-6]     ]
1678884577.7757671 [planner_node-6]   }
1678884577.7758024 [planner_node-6]   durative action navigation(wp o, wp d) {
1678884577.7758374 [planner_node-6]     duration = [10, 10]
1678884577.7758744 [planner_node-6]     conditions = [
1678884577.7759106 [planner_node-6]       [start]:
1678884577.7759442 [planner_node-6]         robot_at(o)
1678884577.7759795 [planner_node-6]     ]
1678884577.7760427 [planner_node-6]     effects = [
1678884577.7761126 [planner_node-6]       end:
1678884577.7761495 [planner_node-6]         robot_at(d) := true:
1678884577.7761836 [planner_node-6]       start:
1678884577.7762163 [planner_node-6]         robot_at(o) := false:
1678884577.7762508 [planner_node-6]     ]
1678884577.7762845 [planner_node-6]     simulated effects = [
1678884577.7763171 [planner_node-6]     ]
1678884577.7763495 [planner_node-6]   }
1678884577.7763817 [planner_node-6] ]
1678884577.7764144 [planner_node-6] 
1678884577.7765701 [planner_node-6] objects = [
1678884577.7766209 [planner_node-6]   door: [door_entrance]
1678884577.7766600 [planner_node-6]   sound: [boiling, doorbell, insect, inside_small_room, mechanical_fan, music, rustle, tubular_bells, white_noise]
1678884577.7766962 [planner_node-6]   wp: [entrance, livingroom]
1678884577.7767313 [planner_node-6] ]
1678884577.7767661 [planner_node-6] 
1678884577.7768130 [planner_node-6] initial fluents default = [
1678884577.7768567 [planner_node-6]   bool door_at[d0=door, w1=wp] := false
1678884577.7768998 [planner_node-6]   bool door_checked[d0=door] := false
1678884577.7769418 [planner_node-6]   bool robot_at[w0=wp] := false
1678884577.7769835 [planner_node-6]   bool sound_listened[s0=sound] := false
1678884577.7770252 [planner_node-6] ]
1678884577.7770660 [planner_node-6] 
1678884577.7771068 [planner_node-6] initial values = [
1678884577.7771471 [planner_node-6]   robot_at(livingroom) := true
1678884577.7771890 [planner_node-6]   door_at(door_entrance, entrance) := true
1678884577.7772298 [planner_node-6]   sound_listened(tubular_bells) := true
1678884577.7772694 [planner_node-6] ]
1678884577.7773125 [planner_node-6] 
1678884577.7773521 [planner_node-6] goals = [
1678884577.7773938 [planner_node-6]   (door_checked(door_entrance) and robot_at(livingroom))
1678884577.7774792 [planner_node-6] ]
1678884577.7775264 [planner_node-6] 
1678884577.7775741 [planner_node-6] 
1678884577.7780237 [planner_node-6] [INFO] [1678884577.775027739] [merlin2.planner_node]: [(Fraction(0, 1), navigation(livingroom, entrance), Fraction(10, 1)), (Fraction(1001, 100), check_door(entrance, door_entrance), Fraction(10, 1)), (Fraction(1001, 100), navigation(entrance, livingroom), Fraction(10, 1))]
1678884577.7783008 [executor_node-8] [INFO] [1678884577.776828442] [merlin2.executor_node]: merlin2_arch_interfaces.srv.GeneratePlan_Response(plan=[merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])], has_solution=True)
1678884577.7783656 [executor_node-8] [INFO] [1678884577.777149872] [merlin2.executor_node]: Plan has solution: True
1678884577.7784219 [executor_node-8] [INFO] [1678884577.777416267] [merlin2.executor_node]: [merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])]
1678884577.8014164 [plan_dispatcher_node-7] [INFO] [1678884577.801176089] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['livingroom', 'entrance']
1678884578.7195942 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884578.7204616 [sound_recognition_node-2] [INFO] [1678884578.720231403] [sound_recognition.sound_recognition_node]: alarm_clock
1678884580.0046661 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884580.0055346 [sound_recognition_node-2] [INFO] [1678884580.005407062] [sound_recognition.sound_recognition_node]: bell
1678884580.0484161 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884580.0497820 [sound_recognition_node-2] [INFO] [1678884580.049492234] [sound_recognition.sound_recognition_node]: vehicle
1678884581.0828433 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884581.0841291 [sound_recognition_node-2] [INFO] [1678884581.083873352] [sound_recognition.sound_recognition_node]: music
1678884582.3525014 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884582.3536935 [sound_recognition_node-2] [INFO] [1678884582.353561880] [sound_recognition.sound_recognition_node]: music
1678884583.6463435 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884583.6471636 [sound_recognition_node-2] [INFO] [1678884583.647013382] [sound_recognition.sound_recognition_node]: vehicle
1678884584.7310882 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884584.7319632 [sound_recognition_node-2] [INFO] [1678884584.731796092] [sound_recognition.sound_recognition_node]: vehicle
1678884586.0069947 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884586.0082140 [sound_recognition_node-2] [INFO] [1678884586.008029948] [sound_recognition.sound_recognition_node]: car
1678884586.0511088 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884586.0525103 [sound_recognition_node-2] [INFO] [1678884586.052294635] [sound_recognition.sound_recognition_node]: music
1678884587.0782769 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884587.0792749 [sound_recognition_node-2] [INFO] [1678884587.079105365] [sound_recognition.sound_recognition_node]: music
1678884588.3589358 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884588.3597465 [sound_recognition_node-2] [INFO] [1678884588.359540684] [sound_recognition.sound_recognition_node]: fire
1678884589.6029940 [plan_dispatcher_node-7] [INFO] [1678884589.602774557] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884589.6080005 [plan_dispatcher_node-7] [INFO] [1678884589.607784180] [merlin2.plan_dispatcher_node]: Executing action check_door with objects ['entrance', 'door_entrance']
1678884589.6557701 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884589.6566753 [sound_recognition_node-2] [INFO] [1678884589.656506238] [sound_recognition.sound_recognition_node]: vehicle
1678884590.7275991 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884590.7283554 [sound_recognition_node-2] [INFO] [1678884590.728173845] [sound_recognition.sound_recognition_node]: vehicle
1678884592.0076108 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0087211 [sound_recognition_node-2] [INFO] [1678884592.008428457] [sound_recognition.sound_recognition_node]: cat
1678884592.0485382 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0494387 [sound_recognition_node-2] [INFO] [1678884592.049249248] [sound_recognition.sound_recognition_node]: purr
1678884593.0732682 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884593.0742242 [sound_recognition_node-2] [INFO] [1678884593.074061453] [sound_recognition.sound_recognition_node]: purr
1678884594.3611791 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884594.3619897 [sound_recognition_node-2] [INFO] [1678884594.361858576] [sound_recognition.sound_recognition_node]: purr
1678884595.6587839 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884595.6597569 [sound_recognition_node-2] [INFO] [1678884595.659593389] [sound_recognition.sound_recognition_node]: purr
1678884596.7353518 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884596.7362726 [sound_recognition_node-2] [INFO] [1678884596.736126401] [sound_recognition.sound_recognition_node]: aircraft
1678884598.0120232 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884598.0135968 [sound_recognition_node-2] [INFO] [1678884598.013389874] [sound_recognition.sound_recognition_node]: vehicle
1678884598.0607984 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 24ms/step
1678884598.0616784 [sound_recognition_node-2] [INFO] [1678884598.061512502] [sound_recognition.sound_recognition_node]: white_noise
1678884598.7223277 [plan_dispatcher_node-7] [INFO] [1678884598.721810188] [merlin2.plan_dispatcher_node]: Action check_door finished
1678884598.7302756 [plan_dispatcher_node-7] [INFO] [1678884598.729979771] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['entrance', 'livingroom']
1678884599.0797648 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884599.0813777 [sound_recognition_node-2] [INFO] [1678884599.081100644] [sound_recognition.sound_recognition_node]: cat
1678884600.3607635 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884600.3616989 [sound_recognition_node-2] [INFO] [1678884600.361469893] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884601.6549842 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884601.6558256 [sound_recognition_node-2] [INFO] [1678884601.655628147] [sound_recognition.sound_recognition_node]: vehicle
1678884602.7287250 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884602.7296121 [sound_recognition_node-2] [INFO] [1678884602.729406425] [sound_recognition.sound_recognition_node]: fireworks
1678884604.0130072 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0138850 [sound_recognition_node-2] [INFO] [1678884604.013727869] [sound_recognition.sound_recognition_node]: vehicle
1678884604.0554757 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0564170 [sound_recognition_node-2] [INFO] [1678884604.056236505] [sound_recognition.sound_recognition_node]: vehicle
1678884605.0930657 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884605.0940287 [sound_recognition_node-2] [INFO] [1678884605.093870245] [sound_recognition.sound_recognition_node]: car
1678884606.3664958 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884606.3674438 [sound_recognition_node-2] [INFO] [1678884606.367253105] [sound_recognition.sound_recognition_node]: speech
1678884607.6561847 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884607.6574214 [sound_recognition_node-2] [INFO] [1678884607.657066928] [sound_recognition.sound_recognition_node]: vehicle
1678884608.7308884 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884608.7318692 [sound_recognition_node-2] [INFO] [1678884608.731702736] [sound_recognition.sound_recognition_node]: door
1678884610.0239010 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884610.0249777 [sound_recognition_node-2] [INFO] [1678884610.024740027] [sound_recognition.sound_recognition_node]: clip-clop
1678884610.0709939 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884610.0720925 [sound_recognition_node-2] [INFO] [1678884610.071893309] [sound_recognition.sound_recognition_node]: vehicle
1678884611.0926340 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884611.0935619 [sound_recognition_node-2] [INFO] [1678884611.093425957] [sound_recognition.sound_recognition_node]: run
1678884612.3709085 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 21ms/step
1678884612.3721375 [sound_recognition_node-2] [INFO] [1678884612.371996360] [sound_recognition.sound_recognition_node]: vehicle
1678884613.6597800 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884613.6606991 [sound_recognition_node-2] [INFO] [1678884613.660547206] [sound_recognition.sound_recognition_node]: fireworks
1678884614.6283243 [plan_dispatcher_node-7] [INFO] [1678884614.628098842] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884614.6424882 [executor_node-8] [INFO] [1678884614.642279934] [merlin2.executor_node]: Removing goals
1678884614.6521719 [merlin2_demo3_node-12] [INFO] [1678884614.651949485] [merlin2.merlin2_demo3_node]: results got
1678884614.6525984 [merlin2_demo3_node-12] [INFO] [1678884614.652343977] [merlin2.merlin2_demo3_node]: True
1678884614.6528592 [merlin2_demo3_node-12] [INFO] [1678884614.652701010] [merlin2.merlin2_demo3_node]: Execution time: 37.00015163421631
1678884614.7444584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884614.7458823 [sound_recognition_node-2] [INFO] [1678884614.745525474] [sound_recognition.sound_recognition_node]: vehicle
1678884615.3285997 [INFO] [merlin2_demo3_node-12]: process has finished cleanly [pid 116658]
1678884616.0222907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884616.0231855 [sound_recognition_node-2] [INFO] [1678884616.023015762] [sound_recognition.sound_recognition_node]: speech
1678884616.0596013 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884616.0607092 [sound_recognition_node-2] [INFO] [1678884616.060568587] [sound_recognition.sound_recognition_node]: animal
1678884617.0980983 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884617.0989578 [sound_recognition_node-2] [INFO] [1678884617.098742894] [sound_recognition.sound_recognition_node]: purr
1678884618.3806093 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884618.3815532 [sound_recognition_node-2] [INFO] [1678884618.381186176] [sound_recognition.sound_recognition_node]: cat
1678884619.6675181 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884619.6683767 [sound_recognition_node-2] [INFO] [1678884619.668243642] [sound_recognition.sound_recognition_node]: white_noise
1678884620.7404547 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884620.7412405 [sound_recognition_node-2] [INFO] [1678884620.741016751] [sound_recognition.sound_recognition_node]: cat
1678884622.0207660 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884622.0216982 [sound_recognition_node-2] [INFO] [1678884622.021457515] [sound_recognition.sound_recognition_node]: fireworks
1678884622.0633199 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884622.0647492 [sound_recognition_node-2] [INFO] [1678884622.064380576] [sound_recognition.sound_recognition_node]: fireworks
1678884623.1012793 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884623.1021008 [sound_recognition_node-2] [INFO] [1678884623.101955993] [sound_recognition.sound_recognition_node]: cat
1678884624.3767979 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884624.3777966 [sound_recognition_node-2] [INFO] [1678884624.377584603] [sound_recognition.sound_recognition_node]: cat
1678884625.6724491 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884625.6735289 [sound_recognition_node-2] [INFO] [1678884625.673325423] [sound_recognition.sound_recognition_node]: cat
1678884626.7613523 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884626.7623341 [sound_recognition_node-2] [INFO] [1678884626.762190369] [sound_recognition.sound_recognition_node]: fireworks
1678884628.0220890 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0229340 [sound_recognition_node-2] [INFO] [1678884628.022791220] [sound_recognition.sound_recognition_node]: animal
1678884628.0623763 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0631883 [sound_recognition_node-2] [INFO] [1678884628.063056020] [sound_recognition.sound_recognition_node]: animal
1678884629.1064036 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884629.1073856 [sound_recognition_node-2] [INFO] [1678884629.107205676] [sound_recognition.sound_recognition_node]: animal
1678884630.3849888 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884630.3859134 [sound_recognition_node-2] [INFO] [1678884630.385733439] [sound_recognition.sound_recognition_node]: cat
1678884631.6770473 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884631.6780236 [sound_recognition_node-2] [INFO] [1678884631.677869932] [sound_recognition.sound_recognition_node]: cat
1678884632.7579663 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884632.7588894 [sound_recognition_node-2] [INFO] [1678884632.758740682] [sound_recognition.sound_recognition_node]: speech
1678884634.0236197 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884634.0247653 [sound_recognition_node-2] [INFO] [1678884634.024479737] [sound_recognition.sound_recognition_node]: fireworks
1678884634.0605907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884634.0614641 [sound_recognition_node-2] [INFO] [1678884634.061317538] [sound_recognition.sound_recognition_node]: fireworks
1678884635.1101820 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884635.1112704 [sound_recognition_node-2] [INFO] [1678884635.111035945] [sound_recognition.sound_recognition_node]: vehicle
1678884636.3903909 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884636.3913989 [sound_recognition_node-2] [INFO] [1678884636.391185251] [sound_recognition.sound_recognition_node]: motorcycle
1678884637.6810584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884637.6820164 [sound_recognition_node-2] [INFO] [1678884637.681732562] [sound_recognition.sound_recognition_node]: stomach_rumble
1678884638.7616808 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884638.7624626 [sound_recognition_node-2] [INFO] [1678884638.762324844] [sound_recognition.sound_recognition_node]: computer_keyboard
1678884639.9263844 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT)
1678884639.9375060 [planner_node-6] [INFO] [1678884639.927608639] [merlin2.planner_node]: Destroying node planner_node
1678884639.9376597 [planner_node-6] Traceback (most recent call last):
1678884639.9377372 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 124, in <module>
1678884639.9378009 [planner_node-6]     main()
1678884639.9378636 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 118, in main
1678884639.9379246 [planner_node-6]     node.join_spin()
1678884639.9379847 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9380448 [planner_node-6]     self._spin_thread.join()
1678884639.9381051 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9381669 [planner_node-6]     self._wait_for_tstate_lock()
1678884639.9382248 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9382832 [planner_node-6]     if lock.acquire(block, timeout):
1678884639.9383414 [planner_node-6] KeyboardInterrupt
1678884639.9386270 [executor_node-8] [INFO] [1678884639.927741220] [merlin2.executor_node]: Destroying node executor_node
1678884639.9387064 [executor_node-8] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9388056 [executor_node-8] Traceback (most recent call last):
1678884639.9388685 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node", line 33, in <module>
1678884639.9389281 [executor_node-8]     sys.exit(load_entry_point('merlin2-executor==0.0.0', 'console_scripts', 'executor_node')())
1678884639.9389863 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/python3.10/site-packages/merlin2_executor/merlin2_executor_node.py", line 101, in main
1678884639.9390466 [executor_node-8]     node.join_spin()
1678884639.9391050 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9391639 [executor_node-8]     self._spin_thread.join()
1678884639.9392228 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9392829 [executor_node-8]     self._wait_for_tstate_lock()
1678884639.9393370 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9393902 [executor_node-8]     if lock.acquire(block, timeout):
1678884639.9394498 [executor_node-8] KeyboardInterrupt
1678884639.9397473 [planner_node-6] [96m[1mNOTE: To disable printing of planning engine credits, add this line to your code: `up.shortcuts.get_environment().credits_stream = None`
1678884639.9397938 [planner_node-6] [0m[96m  *** Credits ***
1678884639.9398353 [planner_node-6] [0m[96m  * In operation mode `OneshotPlanner` at line 72 of `/home/gentlebots/ros2_ws/install/merlin2_planner/local/lib/python3.10/dist-packages/merlin2_planner/merlin2_planners/up_merlin2_planner.py`, [0m[96myou are using the following planning engine:
1678884639.9398808 [planner_node-6] [0m[96m  * Engine name: Tamer
1678884639.9399147 [planner_node-6]   * Developers:  FBK Tamer Development Team
1678884639.9399474 [planner_node-6] [0m[96m  * Description: [0m[96mTamer offers the capability to generate a plan for classical, numerical and temporal problems.
1678884639.9399786 [planner_node-6]   *              For those kind of problems tamer also offers the possibility of validating a submitted plan.[0m[96m
1678884639.9400105 [planner_node-6] [0m[96m
1678884639.9402139 [merlin2_listen_audio_node-9] Traceback (most recent call last):
1678884639.9402971 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node", line 33, in <module>
1678884639.9403560 [merlin2_listen_audio_node-9]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_listen_audio_node')())
1678884639.9404116 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_listen_audio_node.py", line 60, in main
1678884639.9404681 [merlin2_listen_audio_node-9]     rclpy.spin(node_listen)
1678884639.9405236 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9405794 [merlin2_listen_audio_node-9]     executor.spin_once()
1678884639.9406352 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9406912 [merlin2_listen_audio_node-9]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9407454 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9407988 [merlin2_listen_audio_node-9]     return next(self._cb_iter)
1678884639.9408545 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9409101 [merlin2_listen_audio_node-9]     wait_set.wait(timeout_nsec)
1678884639.9409649 [merlin2_listen_audio_node-9] KeyboardInterrupt
1678884639.9412544 [sound_recognition_node-2] Traceback (most recent call last):
1678884639.9413280 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node", line 33, in <module>
1678884639.9413857 [sound_recognition_node-2]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'sound_recognition_node')())
1678884639.9414403 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/sound_recognition_node.py", line 180, in main
1678884639.9414942 [sound_recognition_node-2]     rclpy.spin(sound_recognition_node)
1678884639.9415493 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9416041 [sound_recognition_node-2]     executor.spin_once()
1678884639.9416573 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9417100 [sound_recognition_node-2]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9417644 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9418187 [sound_recognition_node-2]     return next(self._cb_iter)
1678884639.9418733 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9419284 [sound_recognition_node-2]     wait_set.wait(timeout_nsec)
1678884639.9419937 [sound_recognition_node-2] KeyboardInterrupt
1678884639.9422145 [plan_dispatcher_node-7] [INFO] [1678884639.935175976] [merlin2.plan_dispatcher_node]: Destroying node plan_dispatcher_node
1678884639.9422836 [plan_dispatcher_node-7] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9699667 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884639.9701345 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 261, in <module>
1678884639.9705858 [plan_dispatcher_node-7]     main()
1678884639.9707761 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 255, in main
1678884639.9708421 [plan_dispatcher_node-7]     node.join_spin()
1678884639.9708920 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9709430 [plan_dispatcher_node-7]     self._spin_thread.join()
1678884639.9709916 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9710422 [plan_dispatcher_node-7]     self._wait_for_tstate_lock()
1678884639.9710903 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9714367 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884639.9715178 [plan_dispatcher_node-7] KeyboardInterrupt
1678884639.9827285 [waypoint_navigation_node-1] [INFO] [1678884639.982360745] [waypoint_navigation.waypoint_navigation_node]: Destroying node waypoint_navigation_node
1678884639.9828951 [waypoint_navigation_node-1] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0044258 [tts_node-4] [INFO] [1678884640.004114039] [text_to_speech.tts_node]: Destroying node tts_node
1678884640.0055861 [tts_node-4] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0089176 [pddl_generator_node-5] [INFO] [1678884640.008586743] [merlin2.pddl_generator_node]: Destroying node pddl_generator_node
1678884640.0110254 [pddl_generator_node-5] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0383022 [tts_node-4] Traceback (most recent call last):
1678884640.0384836 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node", line 33, in <module>
1678884640.0392134 [tts_node-4]     sys.exit(load_entry_point('text-to-speech==0.0.0', 'console_scripts', 'tts_node')())
1678884640.0393784 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/python3.10/site-packages/text_to_speech/tts_node.py", line 88, in main
1678884640.0398426 [tts_node-4]     node.join_spin()
1678884640.0404348 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0405629 [tts_node-4]     self._spin_thread.join()
1678884640.0406227 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0408790 [tts_node-4]     self._wait_for_tstate_lock()
1678884640.0409479 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0414391 [tts_node-4]     if lock.acquire(block, timeout):
1678884640.0415742 [tts_node-4] KeyboardInterrupt
1678884640.0486207 [manager_node-3] [INFO] [1678884640.048209927] [sound_recognition.manager_node]: Destroying node manager_node
1678884640.0491898 [manager_node-3] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0594249 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.0598230 [executor_node-8] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0599537 [executor_node-8] Traceback (most recent call last):
1678884640.0600307 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0600920 [executor_node-8]     lock.acquire()
1678884640.0601518 [executor_node-8] KeyboardInterrupt: 
1678884640.0606339 [plan_dispatcher_node-7] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f13a644d120>
1678884640.0607460 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884640.0608060 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.0608621 [plan_dispatcher_node-7]     shutdown()
1678884640.0609159 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.0609689 [plan_dispatcher_node-7]     executor.join(1)
1678884640.0610261 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.0610845 [plan_dispatcher_node-7]     self._thread.join(timeout)
1678884640.0611324 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.0614121 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0615094 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0615876 [merlin2_navigation_fsm_action-10]     self._spin_thread.join()
1678884640.0616488 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0617082 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock()
1678884640.0617681 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0621009 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0621994 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0622642 [merlin2_check_door_fsm_action-11]     self._spin_thread.join()
1678884640.0623169 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0626640 [plan_dispatcher_node-7]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.0627830 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0628428 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884640.0628955 [plan_dispatcher_node-7] KeyboardInterrupt: 
1678884640.0631788 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.0632725 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0633259 [merlin2_navigation_fsm_action-10] 
1678884640.0633750 [merlin2_navigation_fsm_action-10] During handling of the above exception, another exception occurred:
1678884640.0634604 [merlin2_navigation_fsm_action-10] 
1678884640.0635068 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0635514 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action", line 33, in <module>
1678884640.0635984 [merlin2_navigation_fsm_action-10]     sys.exit(load_entry_point('merlin2-basic-actions==0.0.0', 'console_scripts', 'merlin2_navigation_fsm_action')())
1678884640.0636446 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/python3.10/site-packages/merlin2_basic_actions/merlin2_navigation_fsm_action.py", line 79, in main
1678884640.0637033 [merlin2_navigation_fsm_action-10]     node.join_spin()
1678884640.0637522 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0638134 [merlin2_navigation_fsm_action-10]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0638635 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0642893 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock()
1678884640.0643778 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0644319 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.0645759 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0646703 [merlin2_check_door_fsm_action-11] 
1678884640.0647247 [merlin2_check_door_fsm_action-11] During handling of the above exception, another exception occurred:
1678884640.0647728 [merlin2_check_door_fsm_action-11] 
1678884640.0648203 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0648930 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action", line 33, in <module>
1678884640.0657759 [merlin2_check_door_fsm_action-11]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_check_door_fsm_action')())
1678884640.0658810 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_check_door_fsm_action.py", line 113, in main
1678884640.0659249 [merlin2_check_door_fsm_action-11]     node.join_spin()
1678884640.0659778 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0660744 [merlin2_check_door_fsm_action-11]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0661254 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0661690 [merlin2_check_door_fsm_action-11]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0662074 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0662374 [merlin2_check_door_fsm_action-11]     caller_id = CallerId()
1678884640.0662651 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0662911 [merlin2_check_door_fsm_action-11]     frame = _find_caller(inspect.currentframe())
1678884640.0663180 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0663452 [merlin2_check_door_fsm_action-11]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0663724 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0665815 [ERROR] [tts_node-4]: process has died [pid 116642, exit code -2, cmd '/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node --ros-args -r __node:=tts_node -r __ns:=/text_to_speech'].
1678884640.0668547 [ERROR] [planner_node-6]: process has died [pid 116646, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node --ros-args -r __node:=planner_node --params-file /tmp/launch_params_7r3e82of'].
1678884640.0670576 [merlin2_navigation_fsm_action-10]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0671303 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0671668 [merlin2_navigation_fsm_action-10]     caller_id = CallerId()
1678884640.0671957 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0672326 [merlin2_navigation_fsm_action-10]     frame = _find_caller(inspect.currentframe())
1678884640.0672596 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0672865 [merlin2_navigation_fsm_action-10]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0673132 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0674167 [ERROR] [merlin2_listen_audio_node-9]: process has died [pid 116652, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node --ros-args -r __node:=listen_audio_node --params-file /tmp/launch_params_2cv5d0ur'].
1678884640.0676262 [sound_recognition_node-2] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0676715 [sound_recognition_node-2] Traceback (most recent call last):
1678884640.0677016 [sound_recognition_node-2]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0677290 [sound_recognition_node-2]     lock.acquire()
1678884640.0677621 [sound_recognition_node-2] KeyboardInterrupt: 
1678884640.0682333 [planner_node-6] [0m
1678884640.0684013 [merlin2_check_door_fsm_action-11]     lines, lnum = findsource(frame)
1678884640.0684705 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0685141 [merlin2_check_door_fsm_action-11]     module = getmodule(object, file)
1678884640.0685487 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0685754 [merlin2_check_door_fsm_action-11]     os.path.realpath(f)] = module.__name__
1678884640.0686009 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 395, in realpath
1678884640.0686257 [merlin2_check_door_fsm_action-11]     path, ok = _joinrealpath(filename[:0], filename, strict, {})
1678884640.0686502 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 430, in _joinrealpath
1678884640.0686753 [merlin2_check_door_fsm_action-11]     st = os.lstat(newpath)
1678884640.0687015 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0688329 [merlin2_navigation_fsm_action-10]     lines, lnum = findsource(frame)
1678884640.0688710 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0688999 [merlin2_navigation_fsm_action-10]     module = getmodule(object, file)
1678884640.0689266 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0689526 [merlin2_navigation_fsm_action-10]     os.path.realpath(f)] = module.__name__
1678884640.0689790 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 396, in realpath
1678884640.0691872 [merlin2_navigation_fsm_action-10]     return abspath(path)
1678884640.0692399 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 385, in abspath
1678884640.0692704 [merlin2_navigation_fsm_action-10]     return normpath(path)
1678884640.0692973 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 370, in normpath
1678884640.0693257 [merlin2_navigation_fsm_action-10]     path = sep.join(comps)
1678884640.0693529 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0708385 [sound_recognition_node-2] terminate called without an active exception
1678884640.0950975 [ERROR] [sound_recognition_node-2]: process has died [pid 116638, exit code -6, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node --ros-args -r __node:=sound_recognition_node -r __ns:=/sound_recognition'].
1678884640.1990383 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.1997647 [merlin2_navigation_fsm_action-10] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.1999891 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.2001505 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2008882 [merlin2_check_door_fsm_action-11] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.2010698 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.2012010 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2017617 [merlin2_navigation_fsm_action-10]     lock.acquire()
1678884640.2019246 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.2024467 [merlin2_check_door_fsm_action-11]     lock.acquire()
1678884640.2026238 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.2085764 [ERROR] [executor_node-8]: process has died [pid 116650, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node --ros-args -r __node:=executor_node --params-file /tmp/launch_params_pm3nbifn'].
1678884640.2101398 [ERROR] [plan_dispatcher_node-7]: process has died [pid 116648, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node --ros-args -r __node:=plan_dispatcher_node --params-file /tmp/launch_params__aeqwv7a'].
1678884640.3144882 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.3149836 [merlin2_check_door_fsm_action-11] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f3a284ffac0>
1678884640.3151383 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.3152375 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3153253 [merlin2_check_door_fsm_action-11]     shutdown()
1678884640.3154082 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3154931 [merlin2_check_door_fsm_action-11]     executor.join(1)
1678884640.3155742 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3156583 [merlin2_check_door_fsm_action-11]     self._thread.join(timeout)
1678884640.3157396 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3162990 [merlin2_navigation_fsm_action-10] Exception ignored in atexit callback: <function _shutdown_resources at 0x7fe101593be0>
1678884640.3164382 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.3165314 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3166242 [merlin2_navigation_fsm_action-10]     shutdown()
1678884640.3167090 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3168330 [merlin2_navigation_fsm_action-10]     executor.join(1)
1678884640.3169751 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3171227 [merlin2_navigation_fsm_action-10]     self._thread.join(timeout)
1678884640.3172050 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3179805 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3181605 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3182542 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.3183537 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.3187332 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3188431 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3189273 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.3190041 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.4113688 [ERROR] [merlin2_check_door_fsm_action-11]: process has died [pid 116656, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action --ros-args -r __node:=check_door --params-file /tmp/launch_params_x5yoc90u'].
1678884640.4120762 [ERROR] [merlin2_navigation_fsm_action-10]: process has died [pid 116654, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action --ros-args -r __node:=navigation --params-file /tmp/launch_params_0i_ko1nb'].
1678884640.4295676 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.5633359 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.6955371 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884641.0691211 [manager_node-3] Traceback (most recent call last):
1678884641.0693920 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0700769 [manager_node-3]     self._spin_thread.join()
1678884641.0702577 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0704384 [manager_node-3]     self._wait_for_tstate_lock()
1678884641.0705881 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0712566 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0713716 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0718808 [waypoint_navigation_node-1]     self._spin_thread.join()
1678884641.0719829 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0721400 [waypoint_navigation_node-1]     self._wait_for_tstate_lock()
1678884641.0722322 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0722940 [waypoint_navigation_node-1]     if lock.acquire(block, timeout):
1678884641.0723536 [waypoint_navigation_node-1] KeyboardInterrupt
1678884641.0724115 [waypoint_navigation_node-1] 
1678884641.0724688 [waypoint_navigation_node-1] During handling of the above exception, another exception occurred:
1678884641.0725276 [waypoint_navigation_node-1] 
1678884641.0725942 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0726573 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node", line 33, in <module>
1678884641.0727687 [waypoint_navigation_node-1]     sys.exit(load_entry_point('waypoint-navigation==0.0.0', 'console_scripts', 'waypoint_navigation_node')())
1678884641.0729141 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/python3.10/site-packages/waypoint_navigation/waypoint_navigation_node.py", line 202, in main
1678884641.0734339 [waypoint_navigation_node-1]     node.join_spin()
1678884641.0735388 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0738482 [manager_node-3]     if lock.acquire(block, timeout):
1678884641.0739362 [manager_node-3] KeyboardInterrupt
1678884641.0740211 [manager_node-3] 
1678884641.0741096 [manager_node-3] During handling of the above exception, another exception occurred:
1678884641.0741870 [manager_node-3] 
1678884641.0742457 [manager_node-3] Traceback (most recent call last):
1678884641.0743215 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node", line 33, in <module>
1678884641.0743973 [manager_node-3]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'manager_node')())
1678884641.0744486 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/manager_node.py", line 111, in main
1678884641.0744917 [manager_node-3]     node.join_spin()
1678884641.0745425 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0746102 [manager_node-3]     self.destroy_node()
1678884641.0746596 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1683, in destroy_node
1678884641.0747027 [manager_node-3]     self.destroy_client(self._clients[0])
1678884641.0747452 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1593, in destroy_client
1678884641.0749857 [waypoint_navigation_node-1]     self.destroy_node()
1678884641.0750623 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884641.0753181 [waypoint_navigation_node-1]     self.destroy_service(self._services[0])
1678884641.0753920 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884641.0756521 [manager_node-3]     client.destroy()
1678884641.0758269 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/client.py", line 187, in destroy
1678884641.0761015 [manager_node-3]     self.__client.destroy_when_not_in_use()
1678884641.0761862 [manager_node-3] KeyboardInterrupt
1678884641.0764089 [waypoint_navigation_node-1]     service.destroy()
1678884641.0764818 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884641.0765414 [waypoint_navigation_node-1]     self.__service.destroy_when_not_in_use()
1678884641.0766015 [waypoint_navigation_node-1] KeyboardInterrupt
1678884642.1252923 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1256349 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884642.1265697 [pddl_generator_node-5]     self._spin_thread.join()
1678884642.1267729 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884642.1268961 [pddl_generator_node-5]     self._wait_for_tstate_lock()
1678884642.1270664 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884642.1277988 [pddl_generator_node-5]     if lock.acquire(block, timeout):
1678884642.1280391 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1282008 [pddl_generator_node-5] 
1678884642.1283841 [pddl_generator_node-5] During handling of the above exception, another exception occurred:
1678884642.1285546 [pddl_generator_node-5] 
1678884642.1286983 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1288023 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 63, in <module>
1678884642.1289310 [pddl_generator_node-5]     main()
1678884642.1290185 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 57, in main
1678884642.1294661 [pddl_generator_node-5]     node.join_spin()
1678884642.1296017 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884642.1300170 [pddl_generator_node-5]     self.destroy_node()
1678884642.1301351 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884642.1302304 [pddl_generator_node-5]     self.destroy_service(self._services[0])
1678884642.1302943 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884642.1306453 [pddl_generator_node-5]     service.destroy()
1678884642.1307805 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884642.1308813 [pddl_generator_node-5]     self.__service.destroy_when_not_in_use()
1678884642.1309750 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1558559 [ERROR] [manager_node-3]: process has died [pid 116640, exit code -2, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node --ros-args -r __node:=manager_node -r __ns:=/sound_recognition'].
1678884642.2004333 [ERROR] [waypoint_navigation_node-1]: process has died [pid 116636, exit code -2, cmd '/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node --ros-args -r __node:=waypoint_navigation_node -r __ns:=/waypoint_navigation --params-file /home/gentlebots/ros2_ws/install/waypoint_navigation/share/waypoint_navigation/params/apartamento_leon.yaml --params-file /tmp/launch_params_ret5a405'].
1678884642.6889017 [ERROR] [pddl_generator_node-5]: process has died [pid 116644, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node --ros-args -r __node:=pddl_generator_node --params-file /tmp/launch_params_l908797v'].

\end{Verbatim}

\end{tiny}

==> assets/launch_log_without_UPF.tex <==

\begin{tiny}

\begin{Verbatim}[breaklines=true, breakanywhere=true]
1678884557.6391342 [INFO] [launch]: All log files can be found below /home/gentlebots/.ros/log/2023-03-15-13-49-17-632183-gentlebots-116634
1678884557.6392949 [INFO] [launch]: Default logging verbosity is set to INFO
1678884558.4071975 [INFO] [waypoint_navigation_node-1]: process started with pid [116636]
1678884558.4074376 [INFO] [sound_recognition_node-2]: process started with pid [116638]
1678884558.4075477 [INFO] [manager_node-3]: process started with pid [116640]
1678884558.4076343 [INFO] [tts_node-4]: process started with pid [116642]
1678884558.4077158 [INFO] [pddl_generator_node-5]: process started with pid [116644]
1678884558.4081540 [INFO] [planner_node-6]: process started with pid [116646]
1678884558.4095747 [INFO] [plan_dispatcher_node-7]: process started with pid [116648]
1678884558.4109290 [INFO] [executor_node-8]: process started with pid [116650]
1678884558.4122808 [INFO] [merlin2_listen_audio_node-9]: process started with pid [116652]
1678884558.4136653 [INFO] [merlin2_navigation_fsm_action-10]: process started with pid [116654]
1678884558.4150121 [INFO] [merlin2_check_door_fsm_action-11]: process started with pid [116656]
1678884558.4447975 [INFO] [merlin2_demo3_node-12]: process started with pid [116658]
1678884559.4909811 [tts_node-4] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6102691 [merlin2_check_door_fsm_action-11] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.6540756 [planner_node-6] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884559.8783755 [manager_node-3] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.1545579 [waypoint_navigation_node-1] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3826396 [executor_node-8] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.3833480 [pddl_generator_node-5] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.4762170 [waypoint_navigation_node-1] /opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py:441: UserWarning: when declaring parameter named 'wps', declaring a parameter only providing its name is deprecated. You have to either:
1678884560.4764743 [waypoint_navigation_node-1] 	- Pass a name and a default value different to "PARAMETER NOT SET" (and optionally a descriptor).
1678884560.4766202 [waypoint_navigation_node-1] 	- Pass a name and a parameter type.
1678884560.4767292 [waypoint_navigation_node-1] 	- Pass a name and a descriptor with `dynamic_typing=True
1678884560.4768608 [waypoint_navigation_node-1]   warnings.warn(
1678884560.4823425 [merlin2_demo3_node-12] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.5726750 [plan_dispatcher_node-7] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6693683 [merlin2_listen_audio_node-9] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884560.6927030 [merlin2_navigation_fsm_action-10] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884561.2024031 [merlin2_demo3_node-12] [INFO] [1678884561.202155833] [merlin2.merlin2_demo3_node]: Waiting for doorbell...
1678884561.2941566 [sound_recognition_node-2] 2023-03-15 13:49:21.293771: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884561.2943850 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884561.5250556 [sound_recognition_node-2] 2023-03-15 13:49:21.524792: I tensorflow/core/util/port.cc:104] oneDNN custom operations are on. You may see slightly different numerical results due to floating-point round-off errors from different computation orders. To turn them off, set the environment variable `TF_ENABLE_ONEDNN_OPTS=0`.
1678884561.5278707 [sound_recognition_node-2] 2023-03-15 13:49:21.527592: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcudart.so.11.0'; dlerror: libcudart.so.11.0: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884561.5280049 [sound_recognition_node-2] 2023-03-15 13:49:21.527611: I tensorflow/compiler/xla/stream_executor/cuda/cudart_stub.cc:29] Ignore above cudart dlerror if you do not have a GPU set up on your machine.
1678884562.4255106 [sound_recognition_node-2] 2023-03-15 13:49:22.425286: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer.so.7'; dlerror: libnvinfer.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4259348 [sound_recognition_node-2] 2023-03-15 13:49:22.425422: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libnvinfer_plugin.so.7'; dlerror: libnvinfer_plugin.so.7: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884562.4260798 [sound_recognition_node-2] 2023-03-15 13:49:22.425431: W tensorflow/compiler/tf2tensorrt/utils/py_utils.cc:38] TF-TRT Warning: Cannot dlopen some TensorRT libraries. If you would like to use Nvidia GPU with TensorRT, please make sure the missing libraries mentioned above are installed properly.
1678884563.2107456 [sound_recognition_node-2] RCUTILS_CONSOLE_STDOUT_LINE_BUFFERED is now ignored. Please set RCUTILS_LOGGING_USE_STDOUT and RCUTILS_LOGGING_BUFFERED_STREAM to control the stream and the buffering of log messages.
1678884563.3666165 [sound_recognition_node-2] 2023-03-15 13:49:23.366304: W tensorflow/compiler/xla/stream_executor/platform/default/dso_loader.cc:64] Could not load dynamic library 'libcuda.so.1'; dlerror: libcuda.so.1: cannot open shared object file: No such file or directory; LD_LIBRARY_PATH: /home/gentlebots/ros2_ws/install/yasmin_demo/lib:/home/gentlebots/ros2_ws/install/yasmin_viewer/lib:/home/gentlebots/ros2_ws/install/yasmin_ros/lib:/home/gentlebots/ros2_ws/install/yasmin_interfaces/lib:/home/gentlebots/ros2_ws/install/yasmin/lib:/home/gentlebots/ros2_ws/install/waypoint_navigation_interfaces/lib:/home/gentlebots/ros2_ws/install/text_to_speech_interfaces/lib:/home/gentlebots/ros2_ws/install/speech_to_text_interfaces/lib:/home/gentlebots/ros2_ws/install/sound_recognition_msgs/lib:/home/gentlebots/ros2_ws/install/kant_dao/lib:/home/gentlebots/ros2_ws/install/kant_knowledge_base/lib:/home/gentlebots/ros2_ws/install/simple_node/lib:/home/gentlebots/ros2_ws/install/merlin2_arch_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_interfaces/lib:/home/gentlebots/ros2_ws/install/kant_dto/lib:/usr/local/lib:/usr/lib/x86_64-linux-gnu/gazebo-11/plugins:/opt/ros/humble/opt/rviz_ogre_vendor/lib:/opt/ros/humble/lib/x86_64-linux-gnu:/opt/ros/humble/lib
1678884563.3667796 [sound_recognition_node-2] 2023-03-15 13:49:23.366321: W tensorflow/compiler/xla/stream_executor/cuda/cuda_driver.cc:265] failed call to cuInit: UNKNOWN ERROR (303)
1678884563.3668425 [sound_recognition_node-2] 2023-03-15 13:49:23.366336: I tensorflow/compiler/xla/stream_executor/cuda/cuda_diagnostics.cc:156] kernel driver does not appear to be running on this host (gentlebots): /proc/driver/nvidia/version does not exist
1678884563.3672061 [sound_recognition_node-2] 2023-03-15 13:49:23.366532: I tensorflow/core/platform/cpu_feature_guard.cc:193] This TensorFlow binary is optimized with oneAPI Deep Neural Network Library (oneDNN) to use the following CPU instructions in performance-critical operations:  AVX2 AVX512F AVX512_VNNI FMA
1678884563.3672807 [sound_recognition_node-2] To enable them in other operations, rebuild TensorFlow with the appropriate compiler flags.
1678884564.7082698 [sound_recognition_node-2] [INFO] [1678884564.708041692] [sound_recognition.sound_recognition_node]: listen_thread starts listening
1678884564.7307980 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.front
1678884564.7310190 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.rear
1678884564.7310867 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.center_lfe
1678884564.7311323 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.side
1678884564.7312636 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313192 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround21
1678884564.7313838 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround40
1678884564.7314229 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround41
1678884564.7318101 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround50
1678884564.7319388 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround51
1678884564.7319987 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.surround71
1678884564.7320669 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321129 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321570 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.iec958
1678884564.7321966 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322392 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.hdmi
1678884564.7322824 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323217 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.modem
1678884564.7323618 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7326291 [sound_recognition_node-2] ALSA lib pcm.c:2664:(snd_pcm_open_noupdate) Unknown PCM cards.pcm.phoneline
1678884564.7371376 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7373369 [sound_recognition_node-2] ALSA lib pcm_oss.c:397:(_snd_pcm_oss_open) Cannot open device /dev/dsp
1678884564.7408085 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7409520 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7410004 [sound_recognition_node-2] ALSA lib confmisc.c:160:(snd_config_get_card) Invalid field card
1678884564.7410374 [sound_recognition_node-2] ALSA lib pcm_usb_stream.c:482:(_snd_pcm_usb_stream_open) Invalid card 'card'
1678884564.7413969 [sound_recognition_node-2] ALSA lib pcm_dmix.c:1032:(snd_pcm_dmix_open) unable to open slave
1678884566.9160802 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 1s 841ms/step
1678884566.9175122 [sound_recognition_node-2] [INFO] [1678884566.917240165] [sound_recognition.sound_recognition_node]: music
1678884567.9730656 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884567.9741521 [sound_recognition_node-2] [INFO] [1678884567.973858829] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884568.0223629 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884568.0231643 [sound_recognition_node-2] [INFO] [1678884568.023020035] [sound_recognition.sound_recognition_node]: insect
1678884569.0709331 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884569.0717046 [sound_recognition_node-2] [INFO] [1678884569.071502259] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884570.3489144 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884570.3496821 [sound_recognition_node-2] [INFO] [1678884570.349498574] [sound_recognition.sound_recognition_node]: boiling
1678884571.6400306 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884571.6410005 [sound_recognition_node-2] [INFO] [1678884571.640862477] [sound_recognition.sound_recognition_node]: white_noise
1678884572.7147002 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884572.7157867 [sound_recognition_node-2] [INFO] [1678884572.715541398] [sound_recognition.sound_recognition_node]: rustle
1678884573.9964857 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884573.9973874 [sound_recognition_node-2] [INFO] [1678884573.997236108] [sound_recognition.sound_recognition_node]: inside_small_room
1678884574.0422242 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884574.0431235 [sound_recognition_node-2] [INFO] [1678884574.042970121] [sound_recognition.sound_recognition_node]: white_noise
1678884575.0656774 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884575.0665801 [sound_recognition_node-2] [INFO] [1678884575.066414965] [sound_recognition.sound_recognition_node]: white_noise
1678884576.3594229 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884576.3607428 [sound_recognition_node-2] [INFO] [1678884576.360408696] [sound_recognition.sound_recognition_node]: inside_small_room
1678884577.6447077 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884577.6457713 [sound_recognition_node-2] [INFO] [1678884577.645569064] [sound_recognition.sound_recognition_node]: tubular_bells
1678884577.6519880 [merlin2_demo3_node-12] [INFO] [1678884577.651800678] [merlin2.merlin2_demo3_node]: EXECUTING MISSION: Answer the door
1678884577.6523142 [merlin2_demo3_node-12] [INFO] [1678884577.652082970] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6556804 [merlin2_demo3_node-12] [INFO] [1678884577.655544354] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6559033 [merlin2_demo3_node-12] [INFO] [1678884577.655777629] [merlin2.merlin2_demo3_node]: Saving goals
1678884577.6604662 [merlin2_demo3_node-12] [INFO] [1678884577.660297157] [merlin2.merlin2_demo3_node]: Saving goals: True
1678884577.6607640 [merlin2_demo3_node-12] [INFO] [1678884577.660550771] [merlin2.merlin2_demo3_node]: goals saved
1678884577.6615767 [merlin2_demo3_node-12] [INFO] [1678884577.661483619] [merlin2.merlin2_demo3_node]: wait for results
1678884577.7237854 [executor_node-8] [INFO] [1678884577.723554341] [merlin2.executor_node]: (define (domain merlin2)
1678884577.7239003 [executor_node-8] (:requirements :typing :negative-preconditions :durative-actions)
1678884577.7239411 [executor_node-8] (:types
1678884577.7239749 [executor_node-8] 	door
1678884577.7240303 [executor_node-8] 	sound
1678884577.7240658 [executor_node-8] 	wp
1678884577.7240963 [executor_node-8] )
1678884577.7241285 [executor_node-8] (:predicates
1678884577.7241755 [executor_node-8] 	(door_at ?d0 - door ?w1 - wp)
1678884577.7242112 [executor_node-8] 	(door_checked ?d0 - door)
1678884577.7242436 [executor_node-8] 	(robot_at ?w0 - wp)
1678884577.7242765 [executor_node-8] 	(sound_listened ?s0 - sound)
1678884577.7243075 [executor_node-8] )
1678884577.7243369 [executor_node-8] (:durative-action check_door
1678884577.7243667 [executor_node-8] 	:parameters ( ?wp - wp ?door - door)
1678884577.7243962 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7244265 [executor_node-8] 	:condition (and
1678884577.7244639 [executor_node-8] 		(at start (door_at ?door ?wp))
1678884577.7245104 [executor_node-8] 		(at start (robot_at ?wp))
1678884577.7245495 [executor_node-8] 	)
1678884577.7245889 [executor_node-8] 	:effect (and
1678884577.7246275 [executor_node-8] 		(at end (door_checked ?door))
1678884577.7246664 [executor_node-8] 	)
1678884577.7247052 [executor_node-8] )
1678884577.7247431 [executor_node-8] (:durative-action navigation
1678884577.7247810 [executor_node-8] 	:parameters ( ?o - wp ?d - wp)
1678884577.7248192 [executor_node-8] 	:duration (= ?duration 10)
1678884577.7248578 [executor_node-8] 	:condition (and
1678884577.7248914 [executor_node-8] 		(at start (robot_at ?o))
1678884577.7249236 [executor_node-8] 	)
1678884577.7249556 [executor_node-8] 	:effect (and
1678884577.7249880 [executor_node-8] 		(at end (robot_at ?d))
1678884577.7250199 [executor_node-8] 		(at start (not (robot_at ?o)))
1678884577.7250516 [executor_node-8] 	)
1678884577.7250829 [executor_node-8] )
1678884577.7251143 [executor_node-8] )
1678884577.7251461 [executor_node-8] 
1678884577.7254245 [executor_node-8] [INFO] [1678884577.723845161] [merlin2.executor_node]: (define (problem merlin2_prb)
1678884577.7254870 [executor_node-8] (:domain merlin2)
1678884577.7255244 [executor_node-8] (:objects
1678884577.7255585 [executor_node-8] 	boiling - sound
1678884577.7255921 [executor_node-8] 	door_entrance - door
1678884577.7256258 [executor_node-8] 	doorbell - sound
1678884577.7256558 [executor_node-8] 	entrance - wp
1678884577.7256918 [executor_node-8] 	insect - sound
1678884577.7257254 [executor_node-8] 	inside_small_room - sound
1678884577.7257576 [executor_node-8] 	livingroom - wp
1678884577.7257905 [executor_node-8] 	mechanical_fan - sound
1678884577.7258232 [executor_node-8] 	music - sound
1678884577.7258549 [executor_node-8] 	rustle - sound
1678884577.7258875 [executor_node-8] 	tubular_bells - sound
1678884577.7259202 [executor_node-8] 	white_noise - sound
1678884577.7259526 [executor_node-8] )
1678884577.7259843 [executor_node-8] (:init
1678884577.7260165 [executor_node-8] 	(robot_at livingroom)
1678884577.7260485 [executor_node-8] 	(door_at door_entrance entrance)
1678884577.7260811 [executor_node-8] 	(sound_listened tubular_bells)
1678884577.7261131 [executor_node-8] )
1678884577.7261448 [executor_node-8] (:goal
1678884577.7261763 [executor_node-8] 	(and
1678884577.7262082 [executor_node-8] 	(door_checked door_entrance)
1678884577.7262411 [executor_node-8] 	(robot_at livingroom)
1678884577.7262723 [executor_node-8] 	)
1678884577.7263045 [executor_node-8] )
1678884577.7263389 [executor_node-8] )
1678884577.7263732 [executor_node-8] 
1678884577.7780237 [planner_node-6] [INFO] [1678884577.775027739] [merlin2.planner_node]: [(Fraction(0, 1), navigation(livingroom, entrance), Fraction(10, 1)), (Fraction(1001, 100), check_door(entrance, door_entrance), Fraction(10, 1)), (Fraction(1001, 100), navigation(entrance, livingroom), Fraction(10, 1))]
1678884577.7783008 [executor_node-8] [INFO] [1678884577.776828442] [merlin2.executor_node]: merlin2_arch_interfaces.srv.GeneratePlan_Response(plan=[merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])], has_solution=True)
1678884577.7783656 [executor_node-8] [INFO] [1678884577.777149872] [merlin2.executor_node]: Plan has solution: True
1678884577.7784219 [executor_node-8] [INFO] [1678884577.777416267] [merlin2.executor_node]: [merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['livingroom', 'entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='check_door', objects=['entrance', 'door_entrance']), merlin2_arch_interfaces.msg.PlanAction(action_name='navigation', objects=['entrance', 'livingroom'])]
1678884577.8014164 [plan_dispatcher_node-7] [INFO] [1678884577.801176089] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['livingroom', 'entrance']
1678884578.7195942 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884578.7204616 [sound_recognition_node-2] [INFO] [1678884578.720231403] [sound_recognition.sound_recognition_node]: alarm_clock
1678884580.0046661 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884580.0055346 [sound_recognition_node-2] [INFO] [1678884580.005407062] [sound_recognition.sound_recognition_node]: bell
1678884580.0484161 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884580.0497820 [sound_recognition_node-2] [INFO] [1678884580.049492234] [sound_recognition.sound_recognition_node]: vehicle
1678884581.0828433 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884581.0841291 [sound_recognition_node-2] [INFO] [1678884581.083873352] [sound_recognition.sound_recognition_node]: music
1678884582.3525014 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884582.3536935 [sound_recognition_node-2] [INFO] [1678884582.353561880] [sound_recognition.sound_recognition_node]: music
1678884583.6463435 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884583.6471636 [sound_recognition_node-2] [INFO] [1678884583.647013382] [sound_recognition.sound_recognition_node]: vehicle
1678884584.7310882 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884584.7319632 [sound_recognition_node-2] [INFO] [1678884584.731796092] [sound_recognition.sound_recognition_node]: vehicle
1678884586.0069947 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884586.0082140 [sound_recognition_node-2] [INFO] [1678884586.008029948] [sound_recognition.sound_recognition_node]: car
1678884586.0511088 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884586.0525103 [sound_recognition_node-2] [INFO] [1678884586.052294635] [sound_recognition.sound_recognition_node]: music
1678884587.0782769 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884587.0792749 [sound_recognition_node-2] [INFO] [1678884587.079105365] [sound_recognition.sound_recognition_node]: music
1678884588.3589358 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884588.3597465 [sound_recognition_node-2] [INFO] [1678884588.359540684] [sound_recognition.sound_recognition_node]: fire
1678884589.6029940 [plan_dispatcher_node-7] [INFO] [1678884589.602774557] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884589.6080005 [plan_dispatcher_node-7] [INFO] [1678884589.607784180] [merlin2.plan_dispatcher_node]: Executing action check_door with objects ['entrance', 'door_entrance']
1678884589.6557701 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884589.6566753 [sound_recognition_node-2] [INFO] [1678884589.656506238] [sound_recognition.sound_recognition_node]: vehicle
1678884590.7275991 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884590.7283554 [sound_recognition_node-2] [INFO] [1678884590.728173845] [sound_recognition.sound_recognition_node]: vehicle
1678884592.0076108 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0087211 [sound_recognition_node-2] [INFO] [1678884592.008428457] [sound_recognition.sound_recognition_node]: cat
1678884592.0485382 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884592.0494387 [sound_recognition_node-2] [INFO] [1678884592.049249248] [sound_recognition.sound_recognition_node]: purr
1678884593.0732682 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884593.0742242 [sound_recognition_node-2] [INFO] [1678884593.074061453] [sound_recognition.sound_recognition_node]: purr
1678884594.3611791 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884594.3619897 [sound_recognition_node-2] [INFO] [1678884594.361858576] [sound_recognition.sound_recognition_node]: purr
1678884595.6587839 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884595.6597569 [sound_recognition_node-2] [INFO] [1678884595.659593389] [sound_recognition.sound_recognition_node]: purr
1678884596.7353518 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884596.7362726 [sound_recognition_node-2] [INFO] [1678884596.736126401] [sound_recognition.sound_recognition_node]: aircraft
1678884598.0120232 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884598.0135968 [sound_recognition_node-2] [INFO] [1678884598.013389874] [sound_recognition.sound_recognition_node]: vehicle
1678884598.0607984 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 24ms/step
1678884598.0616784 [sound_recognition_node-2] [INFO] [1678884598.061512502] [sound_recognition.sound_recognition_node]: white_noise
1678884598.7223277 [plan_dispatcher_node-7] [INFO] [1678884598.721810188] [merlin2.plan_dispatcher_node]: Action check_door finished
1678884598.7302756 [plan_dispatcher_node-7] [INFO] [1678884598.729979771] [merlin2.plan_dispatcher_node]: Executing action navigation with objects ['entrance', 'livingroom']
1678884599.0797648 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884599.0813777 [sound_recognition_node-2] [INFO] [1678884599.081100644] [sound_recognition.sound_recognition_node]: cat
1678884600.3607635 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884600.3616989 [sound_recognition_node-2] [INFO] [1678884600.361469893] [sound_recognition.sound_recognition_node]: mechanical_fan
1678884601.6549842 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884601.6558256 [sound_recognition_node-2] [INFO] [1678884601.655628147] [sound_recognition.sound_recognition_node]: vehicle
1678884602.7287250 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884602.7296121 [sound_recognition_node-2] [INFO] [1678884602.729406425] [sound_recognition.sound_recognition_node]: fireworks
1678884604.0130072 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0138850 [sound_recognition_node-2] [INFO] [1678884604.013727869] [sound_recognition.sound_recognition_node]: vehicle
1678884604.0554757 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884604.0564170 [sound_recognition_node-2] [INFO] [1678884604.056236505] [sound_recognition.sound_recognition_node]: vehicle
1678884605.0930657 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 23ms/step
1678884605.0940287 [sound_recognition_node-2] [INFO] [1678884605.093870245] [sound_recognition.sound_recognition_node]: car
1678884606.3664958 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884606.3674438 [sound_recognition_node-2] [INFO] [1678884606.367253105] [sound_recognition.sound_recognition_node]: speech
1678884607.6561847 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884607.6574214 [sound_recognition_node-2] [INFO] [1678884607.657066928] [sound_recognition.sound_recognition_node]: vehicle
1678884608.7308884 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884608.7318692 [sound_recognition_node-2] [INFO] [1678884608.731702736] [sound_recognition.sound_recognition_node]: door
1678884610.0239010 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884610.0249777 [sound_recognition_node-2] [INFO] [1678884610.024740027] [sound_recognition.sound_recognition_node]: clip-clop
1678884610.0709939 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884610.0720925 [sound_recognition_node-2] [INFO] [1678884610.071893309] [sound_recognition.sound_recognition_node]: vehicle
1678884611.0926340 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884611.0935619 [sound_recognition_node-2] [INFO] [1678884611.093425957] [sound_recognition.sound_recognition_node]: run
1678884612.3709085 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 21ms/step
1678884612.3721375 [sound_recognition_node-2] [INFO] [1678884612.371996360] [sound_recognition.sound_recognition_node]: vehicle
1678884613.6597800 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884613.6606991 [sound_recognition_node-2] [INFO] [1678884613.660547206] [sound_recognition.sound_recognition_node]: fireworks
1678884614.6283243 [plan_dispatcher_node-7] [INFO] [1678884614.628098842] [merlin2.plan_dispatcher_node]: Action navigation finished
1678884614.6424882 [executor_node-8] [INFO] [1678884614.642279934] [merlin2.executor_node]: Removing goals
1678884614.6521719 [merlin2_demo3_node-12] [INFO] [1678884614.651949485] [merlin2.merlin2_demo3_node]: results got
1678884614.6525984 [merlin2_demo3_node-12] [INFO] [1678884614.652343977] [merlin2.merlin2_demo3_node]: True
1678884614.6528592 [merlin2_demo3_node-12] [INFO] [1678884614.652701010] [merlin2.merlin2_demo3_node]: Execution time: 37.00015163421631
1678884614.7444584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 22ms/step
1678884614.7458823 [sound_recognition_node-2] [INFO] [1678884614.745525474] [sound_recognition.sound_recognition_node]: vehicle
1678884615.3285997 [INFO] [merlin2_demo3_node-12]: process has finished cleanly [pid 116658]
1678884616.0222907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884616.0231855 [sound_recognition_node-2] [INFO] [1678884616.023015762] [sound_recognition.sound_recognition_node]: speech
1678884616.0596013 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884616.0607092 [sound_recognition_node-2] [INFO] [1678884616.060568587] [sound_recognition.sound_recognition_node]: animal
1678884617.0980983 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884617.0989578 [sound_recognition_node-2] [INFO] [1678884617.098742894] [sound_recognition.sound_recognition_node]: purr
1678884618.3806093 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 19ms/step
1678884618.3815532 [sound_recognition_node-2] [INFO] [1678884618.381186176] [sound_recognition.sound_recognition_node]: cat
1678884619.6675181 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884619.6683767 [sound_recognition_node-2] [INFO] [1678884619.668243642] [sound_recognition.sound_recognition_node]: white_noise
1678884620.7404547 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884620.7412405 [sound_recognition_node-2] [INFO] [1678884620.741016751] [sound_recognition.sound_recognition_node]: cat
1678884622.0207660 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884622.0216982 [sound_recognition_node-2] [INFO] [1678884622.021457515] [sound_recognition.sound_recognition_node]: fireworks
1678884622.0633199 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 20ms/step
1678884622.0647492 [sound_recognition_node-2] [INFO] [1678884622.064380576] [sound_recognition.sound_recognition_node]: fireworks
1678884623.1012793 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884623.1021008 [sound_recognition_node-2] [INFO] [1678884623.101955993] [sound_recognition.sound_recognition_node]: cat
1678884624.3767979 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884624.3777966 [sound_recognition_node-2] [INFO] [1678884624.377584603] [sound_recognition.sound_recognition_node]: cat
1678884625.6724491 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884625.6735289 [sound_recognition_node-2] [INFO] [1678884625.673325423] [sound_recognition.sound_recognition_node]: cat
1678884626.7613523 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884626.7623341 [sound_recognition_node-2] [INFO] [1678884626.762190369] [sound_recognition.sound_recognition_node]: fireworks
1678884628.0220890 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0229340 [sound_recognition_node-2] [INFO] [1678884628.022791220] [sound_recognition.sound_recognition_node]: animal
1678884628.0623763 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884628.0631883 [sound_recognition_node-2] [INFO] [1678884628.063056020] [sound_recognition.sound_recognition_node]: animal
1678884629.1064036 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884629.1073856 [sound_recognition_node-2] [INFO] [1678884629.107205676] [sound_recognition.sound_recognition_node]: animal
1678884630.3849888 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884630.3859134 [sound_recognition_node-2] [INFO] [1678884630.385733439] [sound_recognition.sound_recognition_node]: cat
1678884631.6770473 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884631.6780236 [sound_recognition_node-2] [INFO] [1678884631.677869932] [sound_recognition.sound_recognition_node]: cat
1678884632.7579663 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884632.7588894 [sound_recognition_node-2] [INFO] [1678884632.758740682] [sound_recognition.sound_recognition_node]: speech
1678884634.0236197 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884634.0247653 [sound_recognition_node-2] [INFO] [1678884634.024479737] [sound_recognition.sound_recognition_node]: fireworks
1678884634.0605907 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884634.0614641 [sound_recognition_node-2] [INFO] [1678884634.061317538] [sound_recognition.sound_recognition_node]: fireworks
1678884635.1101820 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 16ms/step
1678884635.1112704 [sound_recognition_node-2] [INFO] [1678884635.111035945] [sound_recognition.sound_recognition_node]: vehicle
1678884636.3903909 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884636.3913989 [sound_recognition_node-2] [INFO] [1678884636.391185251] [sound_recognition.sound_recognition_node]: motorcycle
1678884637.6810584 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 17ms/step
1678884637.6820164 [sound_recognition_node-2] [INFO] [1678884637.681732562] [sound_recognition.sound_recognition_node]: stomach_rumble
1678884638.7616808 [sound_recognition_node-2] 
1/1 [==============================] - ETA: 0s
1/1 [==============================] - 0s 18ms/step
1678884638.7624626 [sound_recognition_node-2] [INFO] [1678884638.762324844] [sound_recognition.sound_recognition_node]: computer_keyboard
1678884639.9263844 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT)
1678884639.9375060 [planner_node-6] [INFO] [1678884639.927608639] [merlin2.planner_node]: Destroying node planner_node
1678884639.9376597 [planner_node-6] Traceback (most recent call last):
1678884639.9377372 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 124, in <module>
1678884639.9378009 [planner_node-6]     main()
1678884639.9378636 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node", line 118, in main
1678884639.9379246 [planner_node-6]     node.join_spin()
1678884639.9379847 [planner_node-6]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9380448 [planner_node-6]     self._spin_thread.join()
1678884639.9381051 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9381669 [planner_node-6]     self._wait_for_tstate_lock()
1678884639.9382248 [planner_node-6]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9382832 [planner_node-6]     if lock.acquire(block, timeout):
1678884639.9383414 [planner_node-6] KeyboardInterrupt
1678884639.9386270 [executor_node-8] [INFO] [1678884639.927741220] [merlin2.executor_node]: Destroying node executor_node
1678884639.9387064 [executor_node-8] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9388056 [executor_node-8] Traceback (most recent call last):
1678884639.9388685 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node", line 33, in <module>
1678884639.9389281 [executor_node-8]     sys.exit(load_entry_point('merlin2-executor==0.0.0', 'console_scripts', 'executor_node')())
1678884639.9389863 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/merlin2_executor/lib/python3.10/site-packages/merlin2_executor/merlin2_executor_node.py", line 101, in main
1678884639.9390466 [executor_node-8]     node.join_spin()
1678884639.9391050 [executor_node-8]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9391639 [executor_node-8]     self._spin_thread.join()
1678884639.9392228 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9392829 [executor_node-8]     self._wait_for_tstate_lock()
1678884639.9393370 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9393902 [executor_node-8]     if lock.acquire(block, timeout):
1678884639.9394498 [executor_node-8] KeyboardInterrupt
1678884639.9397473 [planner_node-6] [96m[1mNOTE: To disable printing of planning engine credits, add this line to your code: `up.shortcuts.get_environment().credits_stream = None`
1678884639.9397938 [planner_node-6] [0m[96m  *** Credits ***
1678884639.9398353 [planner_node-6] [0m[96m  * In operation mode `OneshotPlanner` at line 72 of `/home/gentlebots/ros2_ws/install/merlin2_planner/local/lib/python3.10/dist-packages/merlin2_planner/merlin2_planners/up_merlin2_planner.py`, [0m[96myou are using the following planning engine:
1678884639.9398808 [planner_node-6] [0m[96m  * Engine name: Tamer
1678884639.9399147 [planner_node-6]   * Developers:  FBK Tamer Development Team
1678884639.9399474 [planner_node-6] [0m[96m  * Description: [0m[96mTamer offers the capability to generate a plan for classical, numerical and temporal problems.
1678884639.9399786 [planner_node-6]   *              For those kind of problems tamer also offers the possibility of validating a submitted plan.[0m[96m
1678884639.9400105 [planner_node-6] [0m[96m
1678884639.9402139 [merlin2_listen_audio_node-9] Traceback (most recent call last):
1678884639.9402971 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node", line 33, in <module>
1678884639.9403560 [merlin2_listen_audio_node-9]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_listen_audio_node')())
1678884639.9404116 [merlin2_listen_audio_node-9]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_listen_audio_node.py", line 60, in main
1678884639.9404681 [merlin2_listen_audio_node-9]     rclpy.spin(node_listen)
1678884639.9405236 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9405794 [merlin2_listen_audio_node-9]     executor.spin_once()
1678884639.9406352 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9406912 [merlin2_listen_audio_node-9]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9407454 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9407988 [merlin2_listen_audio_node-9]     return next(self._cb_iter)
1678884639.9408545 [merlin2_listen_audio_node-9]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9409101 [merlin2_listen_audio_node-9]     wait_set.wait(timeout_nsec)
1678884639.9409649 [merlin2_listen_audio_node-9] KeyboardInterrupt
1678884639.9412544 [sound_recognition_node-2] Traceback (most recent call last):
1678884639.9413280 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node", line 33, in <module>
1678884639.9413857 [sound_recognition_node-2]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'sound_recognition_node')())
1678884639.9414403 [sound_recognition_node-2]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/sound_recognition_node.py", line 180, in main
1678884639.9414942 [sound_recognition_node-2]     rclpy.spin(sound_recognition_node)
1678884639.9415493 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/__init__.py", line 222, in spin
1678884639.9416041 [sound_recognition_node-2]     executor.spin_once()
1678884639.9416573 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 705, in spin_once
1678884639.9417100 [sound_recognition_node-2]     handler, entity, node = self.wait_for_ready_callbacks(timeout_sec=timeout_sec)
1678884639.9417644 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 691, in wait_for_ready_callbacks
1678884639.9418187 [sound_recognition_node-2]     return next(self._cb_iter)
1678884639.9418733 [sound_recognition_node-2]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/executors.py", line 588, in _wait_for_ready_callbacks
1678884639.9419284 [sound_recognition_node-2]     wait_set.wait(timeout_nsec)
1678884639.9419937 [sound_recognition_node-2] KeyboardInterrupt
1678884639.9422145 [plan_dispatcher_node-7] [INFO] [1678884639.935175976] [merlin2.plan_dispatcher_node]: Destroying node plan_dispatcher_node
1678884639.9422836 [plan_dispatcher_node-7] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884639.9699667 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884639.9701345 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 261, in <module>
1678884639.9705858 [plan_dispatcher_node-7]     main()
1678884639.9707761 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node", line 255, in main
1678884639.9708421 [plan_dispatcher_node-7]     node.join_spin()
1678884639.9708920 [plan_dispatcher_node-7]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884639.9709430 [plan_dispatcher_node-7]     self._spin_thread.join()
1678884639.9709916 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884639.9710422 [plan_dispatcher_node-7]     self._wait_for_tstate_lock()
1678884639.9710903 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884639.9714367 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884639.9715178 [plan_dispatcher_node-7] KeyboardInterrupt
1678884639.9827285 [waypoint_navigation_node-1] [INFO] [1678884639.982360745] [waypoint_navigation.waypoint_navigation_node]: Destroying node waypoint_navigation_node
1678884639.9828951 [waypoint_navigation_node-1] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0044258 [tts_node-4] [INFO] [1678884640.004114039] [text_to_speech.tts_node]: Destroying node tts_node
1678884640.0055861 [tts_node-4] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0089176 [pddl_generator_node-5] [INFO] [1678884640.008586743] [merlin2.pddl_generator_node]: Destroying node pddl_generator_node
1678884640.0110254 [pddl_generator_node-5] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0383022 [tts_node-4] Traceback (most recent call last):
1678884640.0384836 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node", line 33, in <module>
1678884640.0392134 [tts_node-4]     sys.exit(load_entry_point('text-to-speech==0.0.0', 'console_scripts', 'tts_node')())
1678884640.0393784 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/text_to_speech/lib/python3.10/site-packages/text_to_speech/tts_node.py", line 88, in main
1678884640.0398426 [tts_node-4]     node.join_spin()
1678884640.0404348 [tts_node-4]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0405629 [tts_node-4]     self._spin_thread.join()
1678884640.0406227 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0408790 [tts_node-4]     self._wait_for_tstate_lock()
1678884640.0409479 [tts_node-4]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0414391 [tts_node-4]     if lock.acquire(block, timeout):
1678884640.0415742 [tts_node-4] KeyboardInterrupt
1678884640.0486207 [manager_node-3] [INFO] [1678884640.048209927] [sound_recognition.manager_node]: Destroying node manager_node
1678884640.0491898 [manager_node-3] Failed to publish log message to rosout: publisher's context is invalid, at ./src/rcl/publisher.c:389
1678884640.0594249 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.0598230 [executor_node-8] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0599537 [executor_node-8] Traceback (most recent call last):
1678884640.0600307 [executor_node-8]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0600920 [executor_node-8]     lock.acquire()
1678884640.0601518 [executor_node-8] KeyboardInterrupt: 
1678884640.0606339 [plan_dispatcher_node-7] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f13a644d120>
1678884640.0607460 [plan_dispatcher_node-7] Traceback (most recent call last):
1678884640.0608060 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.0608621 [plan_dispatcher_node-7]     shutdown()
1678884640.0609159 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.0609689 [plan_dispatcher_node-7]     executor.join(1)
1678884640.0610261 [plan_dispatcher_node-7]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.0610845 [plan_dispatcher_node-7]     self._thread.join(timeout)
1678884640.0611324 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.0614121 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0615094 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0615876 [merlin2_navigation_fsm_action-10]     self._spin_thread.join()
1678884640.0616488 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0617082 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock()
1678884640.0617681 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0621009 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0621994 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884640.0622642 [merlin2_check_door_fsm_action-11]     self._spin_thread.join()
1678884640.0623169 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884640.0626640 [plan_dispatcher_node-7]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.0627830 [plan_dispatcher_node-7]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0628428 [plan_dispatcher_node-7]     if lock.acquire(block, timeout):
1678884640.0628955 [plan_dispatcher_node-7] KeyboardInterrupt: 
1678884640.0631788 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.0632725 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0633259 [merlin2_navigation_fsm_action-10] 
1678884640.0633750 [merlin2_navigation_fsm_action-10] During handling of the above exception, another exception occurred:
1678884640.0634604 [merlin2_navigation_fsm_action-10] 
1678884640.0635068 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.0635514 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action", line 33, in <module>
1678884640.0635984 [merlin2_navigation_fsm_action-10]     sys.exit(load_entry_point('merlin2-basic-actions==0.0.0', 'console_scripts', 'merlin2_navigation_fsm_action')())
1678884640.0636446 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/python3.10/site-packages/merlin2_basic_actions/merlin2_navigation_fsm_action.py", line 79, in main
1678884640.0637033 [merlin2_navigation_fsm_action-10]     node.join_spin()
1678884640.0637522 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0638134 [merlin2_navigation_fsm_action-10]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0638635 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0642893 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock()
1678884640.0643778 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.0644319 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.0645759 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0646703 [merlin2_check_door_fsm_action-11] 
1678884640.0647247 [merlin2_check_door_fsm_action-11] During handling of the above exception, another exception occurred:
1678884640.0647728 [merlin2_check_door_fsm_action-11] 
1678884640.0648203 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.0648930 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action", line 33, in <module>
1678884640.0657759 [merlin2_check_door_fsm_action-11]     sys.exit(load_entry_point('merlin2-demo==0.0.0', 'console_scripts', 'merlin2_check_door_fsm_action')())
1678884640.0658810 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/merlin2_demo/lib/python3.10/site-packages/merlin2_demo/merlin2_check_door_fsm_action.py", line 113, in main
1678884640.0659249 [merlin2_check_door_fsm_action-11]     node.join_spin()
1678884640.0659778 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 61, in join_spin
1678884640.0660744 [merlin2_check_door_fsm_action-11]     self.get_logger().info("Destroying node " + self.get_name())
1678884640.0661254 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 329, in info
1678884640.0661690 [merlin2_check_door_fsm_action-11]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0662074 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0662374 [merlin2_check_door_fsm_action-11]     caller_id = CallerId()
1678884640.0662651 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0662911 [merlin2_check_door_fsm_action-11]     frame = _find_caller(inspect.currentframe())
1678884640.0663180 [merlin2_check_door_fsm_action-11]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0663452 [merlin2_check_door_fsm_action-11]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0663724 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0665815 [ERROR] [tts_node-4]: process has died [pid 116642, exit code -2, cmd '/home/gentlebots/ros2_ws/install/text_to_speech/lib/text_to_speech/tts_node --ros-args -r __node:=tts_node -r __ns:=/text_to_speech'].
1678884640.0668547 [ERROR] [planner_node-6]: process has died [pid 116646, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_planner/lib/merlin2_planner/planner_node --ros-args -r __node:=planner_node --params-file /tmp/launch_params_7r3e82of'].
1678884640.0670576 [merlin2_navigation_fsm_action-10]     return self.log(message, LoggingSeverity.INFO, **kwargs)
1678884640.0671303 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 287, in log
1678884640.0671668 [merlin2_navigation_fsm_action-10]     caller_id = CallerId()
1678884640.0671957 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 59, in __new__
1678884640.0672326 [merlin2_navigation_fsm_action-10]     frame = _find_caller(inspect.currentframe())
1678884640.0672596 [merlin2_navigation_fsm_action-10]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/impl/rcutils_logger.py", line 47, in _find_caller
1678884640.0672865 [merlin2_navigation_fsm_action-10]     file_path = os.path.realpath(inspect.getframeinfo(frame).filename)
1678884640.0673132 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 1629, in getframeinfo
1678884640.0674167 [ERROR] [merlin2_listen_audio_node-9]: process has died [pid 116652, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_listen_audio_node --ros-args -r __node:=listen_audio_node --params-file /tmp/launch_params_2cv5d0ur'].
1678884640.0676262 [sound_recognition_node-2] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.0676715 [sound_recognition_node-2] Traceback (most recent call last):
1678884640.0677016 [sound_recognition_node-2]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.0677290 [sound_recognition_node-2]     lock.acquire()
1678884640.0677621 [sound_recognition_node-2] KeyboardInterrupt: 
1678884640.0682333 [planner_node-6] [0m
1678884640.0684013 [merlin2_check_door_fsm_action-11]     lines, lnum = findsource(frame)
1678884640.0684705 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0685141 [merlin2_check_door_fsm_action-11]     module = getmodule(object, file)
1678884640.0685487 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0685754 [merlin2_check_door_fsm_action-11]     os.path.realpath(f)] = module.__name__
1678884640.0686009 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 395, in realpath
1678884640.0686257 [merlin2_check_door_fsm_action-11]     path, ok = _joinrealpath(filename[:0], filename, strict, {})
1678884640.0686502 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/posixpath.py", line 430, in _joinrealpath
1678884640.0686753 [merlin2_check_door_fsm_action-11]     st = os.lstat(newpath)
1678884640.0687015 [merlin2_check_door_fsm_action-11] KeyboardInterrupt
1678884640.0688329 [merlin2_navigation_fsm_action-10]     lines, lnum = findsource(frame)
1678884640.0688710 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 952, in findsource
1678884640.0688999 [merlin2_navigation_fsm_action-10]     module = getmodule(object, file)
1678884640.0689266 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/inspect.py", line 878, in getmodule
1678884640.0689526 [merlin2_navigation_fsm_action-10]     os.path.realpath(f)] = module.__name__
1678884640.0689790 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 396, in realpath
1678884640.0691872 [merlin2_navigation_fsm_action-10]     return abspath(path)
1678884640.0692399 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 385, in abspath
1678884640.0692704 [merlin2_navigation_fsm_action-10]     return normpath(path)
1678884640.0692973 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/posixpath.py", line 370, in normpath
1678884640.0693257 [merlin2_navigation_fsm_action-10]     path = sep.join(comps)
1678884640.0693529 [merlin2_navigation_fsm_action-10] KeyboardInterrupt
1678884640.0708385 [sound_recognition_node-2] terminate called without an active exception
1678884640.0950975 [ERROR] [sound_recognition_node-2]: process has died [pid 116638, exit code -6, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/sound_recognition_node --ros-args -r __node:=sound_recognition_node -r __ns:=/sound_recognition'].
1678884640.1990383 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.1997647 [merlin2_navigation_fsm_action-10] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.1999891 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.2001505 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2008882 [merlin2_check_door_fsm_action-11] Exception ignored in: <module 'threading' from '/usr/lib/python3.10/threading.py'>
1678884640.2010698 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.2012010 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1567, in _shutdown
1678884640.2017617 [merlin2_navigation_fsm_action-10]     lock.acquire()
1678884640.2019246 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.2024467 [merlin2_check_door_fsm_action-11]     lock.acquire()
1678884640.2026238 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.2085764 [ERROR] [executor_node-8]: process has died [pid 116650, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_executor/lib/merlin2_executor/executor_node --ros-args -r __node:=executor_node --params-file /tmp/launch_params_pm3nbifn'].
1678884640.2101398 [ERROR] [plan_dispatcher_node-7]: process has died [pid 116648, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_plan_dispatcher/lib/merlin2_plan_dispatcher/plan_dispatcher_node --ros-args -r __node:=plan_dispatcher_node --params-file /tmp/launch_params__aeqwv7a'].
1678884640.3144882 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.3149836 [merlin2_check_door_fsm_action-11] Exception ignored in atexit callback: <function _shutdown_resources at 0x7f3a284ffac0>
1678884640.3151383 [merlin2_check_door_fsm_action-11] Traceback (most recent call last):
1678884640.3152375 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3153253 [merlin2_check_door_fsm_action-11]     shutdown()
1678884640.3154082 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3154931 [merlin2_check_door_fsm_action-11]     executor.join(1)
1678884640.3155742 [merlin2_check_door_fsm_action-11]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3156583 [merlin2_check_door_fsm_action-11]     self._thread.join(timeout)
1678884640.3157396 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3162990 [merlin2_navigation_fsm_action-10] Exception ignored in atexit callback: <function _shutdown_resources at 0x7fe101593be0>
1678884640.3164382 [merlin2_navigation_fsm_action-10] Traceback (most recent call last):
1678884640.3165314 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/monitor.py", line 437, in _shutdown_resources
1678884640.3166242 [merlin2_navigation_fsm_action-10]     shutdown()
1678884640.3167090 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 182, in _shutdown_executors
1678884640.3168330 [merlin2_navigation_fsm_action-10]     executor.join(1)
1678884640.3169751 [merlin2_navigation_fsm_action-10]   File "/home/gentlebots/.local/lib/python3.10/site-packages/pymongo/periodic_executor.py", line 100, in join
1678884640.3171227 [merlin2_navigation_fsm_action-10]     self._thread.join(timeout)
1678884640.3172050 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1100, in join
1678884640.3179805 [merlin2_check_door_fsm_action-11]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3181605 [merlin2_check_door_fsm_action-11]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3182542 [merlin2_check_door_fsm_action-11]     if lock.acquire(block, timeout):
1678884640.3183537 [merlin2_check_door_fsm_action-11] KeyboardInterrupt: 
1678884640.3187332 [merlin2_navigation_fsm_action-10]     self._wait_for_tstate_lock(timeout=max(timeout, 0))
1678884640.3188431 [merlin2_navigation_fsm_action-10]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884640.3189273 [merlin2_navigation_fsm_action-10]     if lock.acquire(block, timeout):
1678884640.3190041 [merlin2_navigation_fsm_action-10] KeyboardInterrupt: 
1678884640.4113688 [ERROR] [merlin2_check_door_fsm_action-11]: process has died [pid 116656, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_demo/lib/merlin2_demo/merlin2_check_door_fsm_action --ros-args -r __node:=check_door --params-file /tmp/launch_params_x5yoc90u'].
1678884640.4120762 [ERROR] [merlin2_navigation_fsm_action-10]: process has died [pid 116654, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_basic_actions/lib/merlin2_basic_actions/merlin2_navigation_fsm_action --ros-args -r __node:=navigation --params-file /tmp/launch_params_0i_ko1nb'].
1678884640.4295676 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.5633359 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884640.6955371 [WARNING] [launch]: user interrupted with ctrl-c (SIGINT) again, ignoring...
1678884641.0691211 [manager_node-3] Traceback (most recent call last):
1678884641.0693920 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0700769 [manager_node-3]     self._spin_thread.join()
1678884641.0702577 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0704384 [manager_node-3]     self._wait_for_tstate_lock()
1678884641.0705881 [manager_node-3]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0712566 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0713716 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884641.0718808 [waypoint_navigation_node-1]     self._spin_thread.join()
1678884641.0719829 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884641.0721400 [waypoint_navigation_node-1]     self._wait_for_tstate_lock()
1678884641.0722322 [waypoint_navigation_node-1]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884641.0722940 [waypoint_navigation_node-1]     if lock.acquire(block, timeout):
1678884641.0723536 [waypoint_navigation_node-1] KeyboardInterrupt
1678884641.0724115 [waypoint_navigation_node-1] 
1678884641.0724688 [waypoint_navigation_node-1] During handling of the above exception, another exception occurred:
1678884641.0725276 [waypoint_navigation_node-1] 
1678884641.0725942 [waypoint_navigation_node-1] Traceback (most recent call last):
1678884641.0726573 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node", line 33, in <module>
1678884641.0727687 [waypoint_navigation_node-1]     sys.exit(load_entry_point('waypoint-navigation==0.0.0', 'console_scripts', 'waypoint_navigation_node')())
1678884641.0729141 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/python3.10/site-packages/waypoint_navigation/waypoint_navigation_node.py", line 202, in main
1678884641.0734339 [waypoint_navigation_node-1]     node.join_spin()
1678884641.0735388 [waypoint_navigation_node-1]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0738482 [manager_node-3]     if lock.acquire(block, timeout):
1678884641.0739362 [manager_node-3] KeyboardInterrupt
1678884641.0740211 [manager_node-3] 
1678884641.0741096 [manager_node-3] During handling of the above exception, another exception occurred:
1678884641.0741870 [manager_node-3] 
1678884641.0742457 [manager_node-3] Traceback (most recent call last):
1678884641.0743215 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node", line 33, in <module>
1678884641.0743973 [manager_node-3]     sys.exit(load_entry_point('sound-recognition==0.0.0', 'console_scripts', 'manager_node')())
1678884641.0744486 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/sound_recognition/lib/python3.10/site-packages/sound_recognition/manager_node.py", line 111, in main
1678884641.0744917 [manager_node-3]     node.join_spin()
1678884641.0745425 [manager_node-3]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884641.0746102 [manager_node-3]     self.destroy_node()
1678884641.0746596 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1683, in destroy_node
1678884641.0747027 [manager_node-3]     self.destroy_client(self._clients[0])
1678884641.0747452 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1593, in destroy_client
1678884641.0749857 [waypoint_navigation_node-1]     self.destroy_node()
1678884641.0750623 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884641.0753181 [waypoint_navigation_node-1]     self.destroy_service(self._services[0])
1678884641.0753920 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884641.0756521 [manager_node-3]     client.destroy()
1678884641.0758269 [manager_node-3]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/client.py", line 187, in destroy
1678884641.0761015 [manager_node-3]     self.__client.destroy_when_not_in_use()
1678884641.0761862 [manager_node-3] KeyboardInterrupt
1678884641.0764089 [waypoint_navigation_node-1]     service.destroy()
1678884641.0764818 [waypoint_navigation_node-1]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884641.0765414 [waypoint_navigation_node-1]     self.__service.destroy_when_not_in_use()
1678884641.0766015 [waypoint_navigation_node-1] KeyboardInterrupt
1678884642.1252923 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1256349 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 58, in join_spin
1678884642.1265697 [pddl_generator_node-5]     self._spin_thread.join()
1678884642.1267729 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1096, in join
1678884642.1268961 [pddl_generator_node-5]     self._wait_for_tstate_lock()
1678884642.1270664 [pddl_generator_node-5]   File "/usr/lib/python3.10/threading.py", line 1116, in _wait_for_tstate_lock
1678884642.1277988 [pddl_generator_node-5]     if lock.acquire(block, timeout):
1678884642.1280391 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1282008 [pddl_generator_node-5] 
1678884642.1283841 [pddl_generator_node-5] During handling of the above exception, another exception occurred:
1678884642.1285546 [pddl_generator_node-5] 
1678884642.1286983 [pddl_generator_node-5] Traceback (most recent call last):
1678884642.1288023 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 63, in <module>
1678884642.1289310 [pddl_generator_node-5]     main()
1678884642.1290185 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node", line 57, in main
1678884642.1294661 [pddl_generator_node-5]     node.join_spin()
1678884642.1296017 [pddl_generator_node-5]   File "/home/gentlebots/ros2_ws/install/simple_node/local/lib/python3.10/dist-packages/simple_node/node.py", line 62, in join_spin
1678884642.1300170 [pddl_generator_node-5]     self.destroy_node()
1678884642.1301351 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1685, in destroy_node
1678884642.1302304 [pddl_generator_node-5]     self.destroy_service(self._services[0])
1678884642.1302943 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/node.py", line 1609, in destroy_service
1678884642.1306453 [pddl_generator_node-5]     service.destroy()
1678884642.1307805 [pddl_generator_node-5]   File "/opt/ros/humble/local/lib/python3.10/dist-packages/rclpy/service.py", line 87, in destroy
1678884642.1308813 [pddl_generator_node-5]     self.__service.destroy_when_not_in_use()
1678884642.1309750 [pddl_generator_node-5] KeyboardInterrupt
1678884642.1558559 [ERROR] [manager_node-3]: process has died [pid 116640, exit code -2, cmd '/home/gentlebots/ros2_ws/install/sound_recognition/lib/sound_recognition/manager_node --ros-args -r __node:=manager_node -r __ns:=/sound_recognition'].
1678884642.2004333 [ERROR] [waypoint_navigation_node-1]: process has died [pid 116636, exit code -2, cmd '/home/gentlebots/ros2_ws/install/waypoint_navigation/lib/waypoint_navigation/waypoint_navigation_node --ros-args -r __node:=waypoint_navigation_node -r __ns:=/waypoint_navigation --params-file /home/gentlebots/ros2_ws/install/waypoint_navigation/share/waypoint_navigation/params/apartamento_leon.yaml --params-file /tmp/launch_params_ret5a405'].
1678884642.6889017 [ERROR] [pddl_generator_node-5]: process has died [pid 116644, exit code -2, cmd '/home/gentlebots/ros2_ws/install/merlin2_pddl_generator/lib/merlin2_pddl_generator/pddl_generator_node --ros-args -r __node:=pddl_generator_node --params-file /tmp/launch_params_l908797v'].

\end{Verbatim}

\end{tiny}
